Multi-gap topological conversion of Euler class via band-node braiding: minimal models, $PT$-linked nodal rings, and chiral heirs

The past few years have seen rapid progress in characterizing topological band structures using symmetry eigenvalue indicated methods. Recently, however, there has been increasing theoretical and experimental interest in multi-gap dependent topological phases that cannot be captured by this paradigm. These topologies arise by braiding band degeneracies that reside between different bands and carry non-Abelian charges due to the presence of either $C_2T$ or $PT$ symmetry, culminating in different invariants such as $\mathbb{Z}$-valued Euler class. Here, we present a universal formulation for Euler phases motivated by their homotopy classification that is related to the Skyrmion-profile of a single unit-vector in three-level systems, and that of two unit-vectors in four-level systems. In addition, upon employing the strategy of systematically building 3D models from a pair of sub-dimensional Euler phases, we show that phase transitions between any two inequivalent Euler phases are mediated by the presence of adjacent (in-gap) nodal rings linked with sub-gap nodal lines, forming trajectories corresponding to the braiding or debraiding of nodal points. The stability of the linked adjacent nodal rings is furthermore demonstrated to be indicated by an Euler class monopole charge matching with its $\mathbb{Z}$-valued linking numbers. We finally also systematically address the conversion of Euler phases into descendant Chern phases upon breaking the $C_2T$ or $PT$ symmetry. All the topological phases discussed in this work are corroborated with explicit minimal lattice models. These models can themselves directly serve as an extra impetus for experimental searches or be employed for theoretical studies, thereby underpinning the upcoming of this nascent pursuit.

==> 3D_embedding_braiding.tex <==






\section{Review of 2D case}
We first start by shortly reviewing the two dimensional case. As we pointed out in Ref.~\cite{bouhon2019nonabelian}, \textcolor{orange}{discuss also spinless $C_2$.}


\subsection{Minimal 2D model}
\textcolor{orange}{Copied from appendix of present paper!!!!!!!!!!!!!!!!!!!!!!!!}
The minimal 2D tight-binding model presented in Methods realizes the centered orthorhombic layer group $c222$ (LG$22$), with point group $D_2 = \{C_{2z},C_{2y},C_{2x}\}$~\cite{ITCE}. There are three orbitals per unit cell, one $s$-wave orbital at Wyckoff position $1a$ ($\phi_A$) and one (real) $p_z$-wave orbital at Wyckoff position $2g$ ($\phi_B,\phi_C$), see Fig.~\ref{fig:2D_minimal_lattice} where the primitive cell is spanned by the Bravais lattice vectors $\boldsymbol{a}_1 = (a \hat{x} + b \hat{y})/2$ and $\boldsymbol{a}_2 = (-a \hat{x} + b \hat{y})/2$.

% %%%%%%%%%%%%%%%%%%%% FIGURE HERE %%%%%%%%%%%%%%%%%%%%
% \begin{figure}[h]
% \centering
% \includegraphics[width=0.9\linewidth]{figs/minimal_lattice.pdf}
% \caption{\textsf{Crystal structure of the minimal 2D tight-binding model discussed in the main text and presented in Methods. The conventional unit cell (centered orthorhombic) is spanned by $a \hat{x}$ and $b\hat{y}$. There are three orbitals per each primitive cell spanned by the primitive vectors $\boldsymbol{a}_1$ and $\boldsymbol{a}_2$, one s-wave orbital labeled $\phi_A$ (blue), and two $p_z$-wave orbitals labeled $\phi_B$ and $\phi_C$ (green). The point group is $D_2 = \{C_{2z},C_{2(11)}\equiv C_{2y},C_{2(1\bar{1})}\equiv C_{2x}\}$ with $C_{2z}$ perpendicular to the basal plane.}}
% \label{fig:2D_minimal_lattice} 
% \end{figure}
% %%%%%%%%%%%%%%%%%%%% FIGURE HERE %%%%%%%%%%%%%%%%%%%%
% minimal_model_parameters.pdf
 
 



The locations of the orbitals within the $n$-th unit cell are $\{\boldsymbol{R}_n+\boldsymbol{r}_{\alpha}\}_{\alpha=A,B,C}$, with $\boldsymbol{r}_A = (0,0)$ for $1a$, and $\boldsymbol{r}_B = (0,u)$ and $\boldsymbol{r}_C = (0,-u)$ for $2g$ (written in the Cartesian frame) with $u<b/2$. The tight-binding model is written in the Bloch state basis 
\begin{equation}
    \vert \phi_{\alpha} , \boldsymbol{k} \rangle = \dfrac{1}{\sqrt{N_{\alpha}}} \sum_{\boldsymbol{R}_n} e^{\imi \boldsymbol{k} \cdot \boldsymbol{R}_n }\vert w , \boldsymbol{R}_n + \boldsymbol{r}_{\alpha} \rangle \,, \;\alpha=A,B,C\,,
\end{equation}
that is the discrete Fourier transform of the Wannier states $\vert w , \boldsymbol{R}_n + \boldsymbol{r}_{\alpha} \rangle$ localized at $\boldsymbol{R}_n + \boldsymbol{r}_{\alpha}$, with $N_{\alpha}$ the number of lattice sites occupied by orbital $\alpha$. 

%%%%%%%%%%%%%%%%%%%% FIGURE HERE %%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\includegraphics[width=0.7\linewidth]{figs/minimal_model_parameters.pdf}
\caption{\textsf{Tight-binding parameters of the 2D minimal model as functions of the control parameter $t$. }}
\label{fig:2D_minimal_parameters} 
\end{figure}
%%%%%%%%%%%%%%%%%%%% FIGURE HERE %%%%%%%%%%%%%%%%%%%%
\textcolor{orange}{End Copied from appendix of present paper!!!!!!!!!!!!!!!!!!!!!!!!}

 The 2D minimal model discussed in Ref.~\cite{bouhon2019nonabelian} can be formulated in terms of the generic tight-binding model as follows.  Since the model is defined within a single basal plane only we introduce the following parameters.
 
 \textcolor{orange}{Start with setup}
, we first set $p^{u,d}_j = 0$ for all $j$. Then, among the basal tight-binding terms only the following are set to finite values $\{a^0_0,d^0_5,d^0_7,f^0_0,f^0_1,f^0_3\}$. 


Importantly, the overly simplified form of the minimal model leads to an effective auxiliary $C_2$ symmetry 
\begin{equation}
\label{eq_C2_bis}
    U (1\oplus \sigma_x) H(C_2\boldsymbol{k}) (1\oplus \sigma_x) U^{\dagger}  = H(\boldsymbol{k}) \;,
\end{equation}
with $U=\mathrm{diag}(-1,1,1)$ corresponding to the gauge transformation $\phi_A\rightarrow -\phi_A$. This can be straightforwardly verified from the explicit expressions Eq.~(\ref{eqn:Ham-matrix_sup}) and (\ref{eq_2}). 

As a consequence of this effective symmetry, the band structure is $C_2$ symmetric and Weyl points (WPs) can only be created four at a time, i.e.~two pairs of WPs with opposite chirality. Indeed, any WP at $\boldsymbol{k}$ must have its symmetric partner of equal chirality at $C_2\boldsymbol{k}$, and these must have their symmetric partners of opposite chirality at $-C_2\boldsymbol{k}$ and $-\boldsymbol{k}$ due to $C_2\mathcal{T}$ symmetry. This property is relaxed in the model used for the 3D protocol of the main text, see Section A7. 

\subsection{Braiding and conversion}
Using free parameters we now discuss the braiding.


Introducing the parameter $t$ that controls the braiding and using the notations of the main text, we obtain the minimal model
\begin{equation}
H_{2D}(\bs{k};t) = \left(\begin{array}{ccc}
f(t)       &   g(\bs{k})      &   g^*(\bs{k})    \\
g^*(\bs{k})    &   0              &   h(\bs{k};t)      \\
g(\bs{k})      &   h^*(\bs{k};t)  &   0   
\end{array}\right)\;, \label{eqn:Ham-matrix_sup} %:)
\end{equation}
where 
\begin{equation}
\label{eq_2}
\begin{aligned}
    f(t) &= a^0_0(t) \;, \\
    g(\bs{k}) &= d^0_5 \e{-\imi k_1 \pi} + d^0_7 \e{-\imi k_2\pi} \;,\\
    %=-\imi(\e{-\imi k_1 \pi}-\e{-\imi k_2\pi})\;,\\
    h(\bs{k};t) &= f^0_0(t) + f^0_1(t) \e{\imi k_1 \pi}+ f^0_3(t)  \e{\imi k_2 \pi} \;,
\end{aligned}
\end{equation}
and
\begin{equation}
\label{eq_3}
    \begin{array}{rclrcl}
        a^0_0(t) &=& F_{[8,-]}(t) \,, & f^0_0(t) &=& F_{[2,-]}(t) \\
        d^0_5 &=& -\imi \,, & f^0_1(t) &=& 10-F_{[8,+]}(t) \,, \\
        d^0_7 &=& \imi \,, & f^0_3(t) &=& f^0_1(t) \,,
    \end{array}
\end{equation}
with the $t$-dependent functions defined through $F_{[\rho,\pm]}(t) = 1/2(\vert t+\nu \vert\pm \vert t-\nu \vert)$, see Fig.~\ref{fig:2D_minimal_parameters}. 





\section{Models for non-Abelian reciprocal braiding in 3D}

\subsection{3D embedding of the minimal 2D model}


The minimal 2D model can be readily embedded into 3D using the above insights. In order to have all bands gapped at $k_3=1$, we set the extra parameter $d^0_0 = 4\imi $, while all the other basal parameters are kept the same as in the 2D case. We remark that this preserves the auxiliary $C_2$ symmetry Eq.~(\ref{eq_C2_bis}) so that WPs must be created or annihilated four at a time.  

In Fig.~\ref{fig:protocol_3D_embedded} we show the 3D embedding of the minimal 2D model at successive snapshots for $t\in[-10,10]$. The 3D band structures are represented through two-dimensional slices taken, in one direction, along the diagonals $(1\bar{1}0)$ and $(110)$ (connecting $\Gamma$ to M), and then $(100)$ (connecting $\Gamma$ to X), successively, and, in the other direction, along $(001)$ for $k_3\in[0,1]$, i.e. along the $C_2$ axis perpendicular to the basal plane. 

We start with the three bands gapped ($t=-10$), then four WPs are created in the second gap at $\Gamma$ ($t=-9$), with two WPs of equal chirality moving towards M along the $(1\bar{1}0)$ diagonal and two WPs with the other chirality located outside the symmetric plane, one above and one underneath $\Gamma$ ($t=-8$). Note that by the effective $C_2$ symmetry, the two WPs above and underneath $\Gamma$ are trapped on the $C_2$ axis crossing $\Gamma$.   

At $t=-4$, two WPs of equal chirality have been created in the first gap at M, above and underneath which we find their two partners of creation. The later are again trapped on the $C_2$ axis crossing M, as imposed by the effective $C_2$ symmetry. The two WPs within the symmetric plane ($k_3=0$) are heading along the diagonal $(110)$ towards $\Gamma$, where they meet at the later time $t=-2$. These do not leave the symmetric plane though, as we find them at $t=0$ moving now along the diagonal $(1\bar{1}0)$. 

At $t=2$, the two WPs of the second gap within the symmetric plane meet at M without leaving the plane, as we can see at $t=4$ where they now move along $(110)$ towards $\Gamma$. At $t=8$, they have reached $\Gamma$ where they recombine and annihilate with their two partners of creation. At $t=9$, the WPs of the first gap within the symmetric plane meet eventually at M where they also recombine and annihilate with their two partners of creation.    


As discussed in the main text, the non-Abelian frame-rotation charge captures the stability of two WPs colliding within a $C_2\mathcal{T}$ symmetric plane. On the hand, we have found above (Fig.~\ref{fig:protocol_3D_embedded}) that equal chirality WPs from one gap bounce away as a consequence of the braiding with the WPs of the adjacent gap. On the other hand, we illustrate the case without braiding in Fig.~\ref{fig:protocol_3D_embedded_bis}. In this case, there is no obstruction for two WPs of equal chirality to leave the symmetric plane after colliding, as can be seen in panel 4. of Fig.~\ref{fig:protocol_3D_embedded_bis}. 

%%%%%%%%%%%%%%%%%%%% FIGURE HERE %%%%%%%%%%%%%%%%%%%%
\begin{figure*}[htpb!]
\centering
\begin{tabular}{llll} 
	\includegraphics[width=0.25\linewidth]{figs/3D__BS_6c.png} &
	\includegraphics[width=0.25\linewidth]{figs/3D__BS_6b.png} &
	\includegraphics[width=0.25\linewidth]{figs/3D__BS_6.png} &
	\includegraphics[width=0.25\linewidth]{figs/3D__BS_5.png} \\
	$1.~t=-10$ &
	$2.~t=-9$ &
    $3.~t=-8$ &
	$4.~t=-4$ \\
	\includegraphics[width=0.25\linewidth]{figs/3D__BS_4.png} &
	\includegraphics[width=0.25\linewidth]{figs/3D__BS_34.png} &
	\includegraphics[width=0.25\linewidth]{figs/3D__BS_3.png} &
	\includegraphics[width=0.25\linewidth]{figs/3D__BS_2.png} \\
	$5.~t=-2$ &
	$6.~t=0$ &
	$7.~t=2$ &
	$8.~t=4$ \\
	\includegraphics[width=0.25\linewidth]{figs/3D__BS_1.png} &
	\includegraphics[width=0.25\linewidth]{figs/3D__BS_1c.png} &
	\includegraphics[width=0.25\linewidth]{figs/3D__BS_1b.png} & \\
	$9.~t=8$ &
	$10.~t=9$ &
	$11.~t=10$ & 
\end{tabular}\\
\caption{\textsf{\textbf{3D embedding of the 2D braiding protocol.} The braiding protocol for the minimal 2D model discussed in the main text is controlled by $t$. This setup can be embedded in 3D so that the 2D nodal points are realized as Weyl points within a single $C_2\mathcal{T}$ symmetric plane ($k_3=0$), and with the three bands gapped on the other symmetric plane ($k_3=1$). We draw the two-dimensional slices of the 3D Band structures with the long direction taken as the diagonals $(1\bar{1}0)$ and $(110)$ (connecting $\Gamma$ to M), and $(100)$ (connecting $\Gamma$ to X), and with the second direction taken as $(001)$, i.e. for $k_3\in[0,1]$ (connecting the two $C_2\mathcal{T}$ symmetric planes). }}
\label{fig:protocol_3D_embedded} 
\end{figure*}
%%%%%%%%%%%%%%%%%%%% FIGURE HERE %%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%% FIGURE HERE %%%%%%%%%%%%%%%%%%%%
\begin{figure*}[htpb!]
\centering
\begin{tabular}{llll} 
	\includegraphics[width=0.25\linewidth]{figs/3D__BS_1.png} &
	\includegraphics[width=0.25\linewidth]{figs/3D__BS_7.png} &
	\includegraphics[width=0.25\linewidth]{figs/3D__BS_7b.png} &
	\includegraphics[width=0.25\linewidth]{figs/3D__BS_8.png} \\
	$1.~t=8$ & 2.& 3.&4. 
\end{tabular}\\
\caption{\textsf{\textbf{3D embedding without braiding.} When there is no braiding two WPs of equal chirality are allowed to leave the symmetric plane after colliding. The two WPs of the first gap created at M meet at $\Gamma$ and leave the symmetric plane along the vertical $C_2$ axis. In the middle of the process, we find that the WPs are converted into a nodal line centered on M that crosses the points X and Y of the Brillouin zone, see panel 2. Then in the tird panel the WPs reappeared on $(1\bar{1}0)$, but four extra WPs have emerged out of the nodal line and populate the two vertical $C_2$ axes crossing X and Y (here only X is shown). Eventually, the two WPs within the symmetric plane meet at $\Gamma$ and leave the plane, see panel 4.}}
\label{fig:protocol_3D_embedded_bis} 
\end{figure*}
%%%%%%%%%%%%%%%%%%%% FIGURE HERE %%%%%%%%%%%%%%%%%%%%

\subsection{Generic tight-binding model}
We derive a generic three-dimensional three-band tight-binding model with the single constraint that it satisfies $C_2\mcT$ symmetry with $(C_2\mcT)^2=+1$, and given a choice of the Wyckoff positions. $C_2\mcT$ symmetry requires the magnetic space group $P12'1$ (\#3.3.10) as minimal subgroup \cite{MITC,BradCrack}, i.e. the direct product between the primitive monoclinic Bravais lattice as the normal subgroup of translations and the magnetic point group $2' = \{E,C_2\mcT\}$ (\#3.3.8) with $\hat{y}$ as the $C_2$ rotation axis \cite{MITC,BradCrack}.  

We choose the primitive lattice vectors as $\boldsymbol{a}_1 = a(\sin \theta,0,\cos \theta)$, $\boldsymbol{a}_2 = b(1,0,0)$, and $\boldsymbol{a}_3 = c(0,1,0)$, and write their dual (primitive reciprocal lattice vectors) as $\{\boldsymbol{b}_1,\boldsymbol{b}_2,\boldsymbol{b}_3\}$ ($\boldsymbol{a}_i \cdot \boldsymbol{b}_j = 2\pi \delta_{ij}$) taken as the basis for the Bloch wave vector (momentum) $\boldsymbol{k} = (k_1 \boldsymbol{b}_1+k_2 \boldsymbol{b}_2+k_3 \boldsymbol{b}_3)/2$. Note that the $C_2$ rotation axis ($\hat{y}$ as in \cite{MITC}) is $\boldsymbol{a}_3$ in our basis, i.e.~it acts component-wise on the momentum as $C_2(k_1,k_2,k_3) = (-k_1,-k_2,k_3)$. The $C_2$ rotation axis defines a basal plane perpendicular to it. 

%We note that t
The advantage of the crystallographic convention ($C_2$ taken along $\hat{y}$) is that if we choose $\hat{z}$ as the quantization axis for the spin, the representation of $C^{(\hat{y})}_{2}\mathcal{T}$ symmetry on the pure spinor basis ($\phi_{\uparrow},\phi_{\downarrow}$) takes the simple form $(-\imi\sigma_y)(\imi\sigma_y \mathcal{K}) = \mathbf{1} \mathcal{K}$ (where $\mathcal{K}$ is complex conjugation), i.e.~it makes explicit the fact that it acts trivially on the spin degrees of freedom. As a consequence, our model below holds both for spinful and spinless systems, since it is constrained only by $C_2\mathcal{T}$ symmetry. Form now on we thus discard spin indices and remark explicitly when a statement is only valid for the spinless case.


In the following we make the assumption that one real $s$-wave orbital sits on Wyckoff's positions $1b$ and $2e$ \cite{MITC}. Since $2e$ is twofold ($1b$ is invariant under $C_2$, $2e$ is not) there are three sub-lattice sites per unit cell. We take their locations within the $n$-th unit cell as $\{\boldsymbol{R}_n+\boldsymbol{r}_{\alpha}\}_{\alpha=A,B,C}$, with $\boldsymbol{r}_A = (0,0,0)$ for $1b$, and $\boldsymbol{r}_B = (u,v,w)$ and $\boldsymbol{r}_C = (-u,-v,w)$ for $2e$ (here and in the following we write all vectors of the direct space in the primitive basis $\{\boldsymbol{a}_i\}_{i=1,2,3}$). We write the localized Wannier function for the $\alpha$-th orbital of the $n$-th unit cell as $\vert w , \boldsymbol{R}_n + \boldsymbol{r}_{\alpha} \rangle$. The Bloch basis is then given through the discrete Fourier transform as 
\begin{equation}
    \vert \varphi_{\alpha} , \boldsymbol{k} \rangle = \dfrac{1}{\sqrt{N_{\alpha}}} \sum_{\boldsymbol{R}_n} e^{\imi \boldsymbol{k} \cdot \boldsymbol{R}_n }\vert w , \boldsymbol{R}_n + \boldsymbol{r}_{\alpha} \rangle \,, \;\alpha=A,B,C\,,
\end{equation}%e^{i \boldsymbol{k} \cdot (\boldsymbol{R}_n + \boldsymbol{r}_{\alpha})}
with $N_{\alpha}$ the number of lattice sites with an $\alpha$-orbital. In the following we use the row vector notation $\vert \boldsymbol{\varphi} , \boldsymbol{k} \rangle = \left(\vert \varphi_A , \boldsymbol{k} \rangle ~ \vert \varphi_B , \boldsymbol{k} \rangle ~\vert \varphi_C , \boldsymbol{k} \rangle\right)$. $C_2 \mathcal{T}$ symmetry acts then as
\begin{equation}
    ^{C_2 \mathcal{T}} \vert \boldsymbol{\varphi} , \boldsymbol{k} \rangle = \vert \boldsymbol{\varphi} , (k_1,k_2,-k_3) \rangle (1\oplus \sigma_x) \mathcal{K} \;.
\end{equation}

We can now write the Bloch tight-binding model
\begin{equation}
    \mathcal{H} = \sum_{\boldsymbol{k}\in \mathrm{BZ}} \vert \boldsymbol{\varphi} , \boldsymbol{k} \rangle H(\boldsymbol{k}) \langle \boldsymbol{\varphi} , \boldsymbol{k} \vert\;,
\end{equation}
with the matrix components
\begin{equation}
\label{eq_TB_parameter}
    H_{\alpha\beta}(\boldsymbol{k}) = 
    \sum_{\boldsymbol{n}\in \mathbb{N}^3} 
    T_{\alpha\beta}(\boldsymbol{n}) e^{\imi \boldsymbol{k}\cdot (n_1 \boldsymbol{a}_1+ n_2 \boldsymbol{a}_2 + n_3 \boldsymbol{a}_3 )}\,,
\end{equation}%e^{i \boldsymbol{k}\cdot (\boldsymbol{r}_{\beta}-\boldsymbol{r}_{\alpha} +
where the Bloch wave vector $\boldsymbol{k}= (k_1 \boldsymbol{b}_1+k_2 \boldsymbol{b}_2+k_3 \boldsymbol{b}_3)/2$ is taken within the first Brillouin zone (BZ), i.e. $(k_{1},k_{2},k_{3})\in (-1,1]^{\times 3}$.  


The hopping parameters $T_{\alpha\beta}(\boldsymbol{n}) \in \mathbb{C}$ are constrained by symmetry. First of all, hermiticity imposes 
\begin{equation}
\label{eq_sym_herm}
    T_{\beta\alpha}(\boldsymbol{n}) = T_{\alpha\beta}(-\boldsymbol{n})^*\,.
\end{equation} 
Then, $C_2\mathcal{T}$ requires 
\begin{equation}
    (1\oplus\sigma_x) H^*(k_1,k_2,k_3) (1\oplus\sigma_x) = H(k_1,k_2,-k_3)\;,
\end{equation}
which can be recast into constraints
\begin{equation}
\label{eq_sym_C2T}
\begin{array}{ll}
      T_{AA}(C_2\boldsymbol{n})=T_{AA}(\boldsymbol{n})^* \,,&  
      T_{AC}(C_2\boldsymbol{n})=T_{AB}(\boldsymbol{n})^* \,,\\
      T_{CC}(C_2\boldsymbol{n})=T_{BB}(\boldsymbol{n})^* \,,&
      T_{CB}(C_2\boldsymbol{n})=T_{BC}(\boldsymbol{n})^* \,.
\end{array}
\end{equation}

In the following we choose the parameters $\{T_{BA}(\boldsymbol{n}),T_{BC}(\boldsymbol{n}),T_{CA}(\boldsymbol{n}),T_{AC}(\boldsymbol{n}),T_{CC}(\boldsymbol{n})\}$ as functions of the other parameters, respecting Eqs.~(\ref{eq_sym_herm}) and~(\ref{eq_sym_C2T}). 

\subsection{Explicit 3D model}

Taking the origin $\boldsymbol{0}$ of the Bravais lattice as a reference, and using $\boldsymbol{n}$ of Eq.~(\ref{eq_TB_parameter}) to label its neighbors, we limit the tight-binding model to the following neighbors: from the basal plane $\boldsymbol{n}_0\in \{ (n_1,n_2,0) \in \mathbb{N}^2 \vert n_1, n_2 = -1,0,1\}$, from the first plane above $\boldsymbol{n}_u \in \{ (n_1,n_2,1) \in \mathbb{N}^2 \vert  n_1, n_2 = -1,0,1 \}$, and the first plane below $\boldsymbol{n}_{d} \in \{ (n_1,n_2,-1) \in \mathbb{N}^2 \vert n_1, n_2 = -1,0,1 \}$. In the following we use `$0$', `$u$', and `$d$' to refer respectively to the basal plane, the upper plane (up), and the lower plane (down).

%%%%%%%%%%%%%%%%%%%% FIGURE HERE %%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\includegraphics[width=1.0\linewidth]{figs/FigSup.jpeg}
\caption{\textsf{Schematic representation of the hopping amplitudes. The 3D model is composed of a three atom basis that is arranged in a simple cubic lattice. Considering the site marked by "$0$", in-plane hopping is denoted by $p^{0}_j$, where $j$ refers to the eight neighbors $1-8$. Similarly,  $p^{d}_j$ and $p^{u}_j$ denote hopping to a layer beneath and above, respectively. The specific arrangement of these parameters is outlined in the text. The basis units are colored differently depending on the layer to further elucidate the crystal structure. }}
\label{fig:3D_hopping} 
\end{figure}
%%%%%%%%%%%%%%%%%%%% FIGURE HERE %%%%%%%%%%%%%%%%%%%%

Let us label the neighbors around within each plane clockwise from $1$ to $8$ as a function of $(n_1,n_2)$, i.e.~$1:(1,0)$, $2:(1,1)$, $3:(0,1)$, $4:(-1,1)$, $5:(-1,0)$, $6:(-1,-1)$, $7:(0,-1)$, $8:(1,-1)$, and $0:(0,0)$, see Fig.~\ref{fig:3D_hopping}. We then use a more compact labeling of the parameters as $\{T_{AA}(\boldsymbol{n}_0)\}_{\boldsymbol{n}_0} = \{a^0_{j} \}_{j=0,\dots,8}$, $\{T_{AA}(\boldsymbol{n}_u)\}_{\boldsymbol{n}_u} = \{a^u_{j }\}_{j=0,\dots,8}$, and $\{T_{AA}(\boldsymbol{n}_{d})\}_{\boldsymbol{n}_{d}} = \{a^{d}_{j}\}_{j=0,\dots,8}$. We proceed similarly for $T_{BB} = b $, $T_{CC} = c $, $T_{AB} = d $, $T_{AC} = e $, and $T_{BC} = f $, while the labeling of $T_{BA}$, $T_{BC}$, and $T_{CA}$ is readily given by hermiticity Eq.~(\ref{eq_sym_herm}). 

We can now rewrite the constraints following from Eq.~(\ref{eq_sym_herm}) and (\ref{eq_sym_C2T}) in terms of the compact labeling, i.e.
$$
c^{\mu}_{j+4} = (b^{\mu}_{j })^* ,  \; c^{\mu}_{j} = (b^{\mu}_{j+4 })^* , \; e^{\mu}_{j+4} = (d^{\mu}_{j })^*,  \;e^{\mu}_{j} = (d^{\mu}_{j +4})^*,
$$
for $j=1,\dots,4$ and $\mu=0,u,d$, and $c^{\mu}_{0} = (b^{\mu}_{0})^*$. Note that since the $c$'s and $e$'s are here all determined by the $b$'s and the $d$'s, respectively, we do not refer to them anymore. Then, 
$$a^d_{j} = a^u_{j}\;,\; f^{d}_j = f^{u}_j  \;, $$ 
for $j=0,\dots,8$, and with $a^u_{0} \in \mathbb{R}$. Furthermore, 
$$a^0_{j+4} = (a^0_{j})^*\;,\;b^0_{j+4} = (b^0_{j})^*  \;, $$ 
for $j=1,\dots,4$, and with $a^0_{0},b^0_{0} \in \mathbb{R}$. Finally, 
$$b^d_{j+4} = (b^u_{j})^*\; , \; b^d_{j} = (b^u_{j+4})^*\;,  $$ 
for $j=1,\dots,4$, and $b^d_{0} = (b^u_{0})^*$. In the following, any parameter that is not explicitly constrained to be real is considered as a complex number.



We note that from the form of Eq.~(\ref{eq_TB_parameter}) the three $p^{0,u,d}_{j}$-terms for fixed $p\in\{a,b,d,f\}$ and $j\in\{1,\dots,8\}$ all have the same $(k_1,k_2)$-dependence. On the one hand, the $p^{0}_{j}$-terms have no $k_3$ dependence. On the other hand, the $p^{u}_{j}$- and $p^{d}_{j}$-terms have the form factors of the $p^{0}_{j}$-terms multiplied respectively by $e^{\imi k_3\pi}$, and by $e^{-\imi k_3\pi}$. As a consequence, a generic 3D model has the form
\begin{equation}
\begin{aligned}
\label{eq_generic_3D}
    H_{3D}[\{p^{0,u,d}_{j}\}_{p,j}](k_1,k_2,k_3) &= H_{2D}[\{p^{0}_{j}\}_{p,j}](k_1,k_2,0) \\ 
    &+ H_{2D}[\{p^{u}_{j}\}_{p,j}](k_1,k_2,k_3) \\
    &+H_{2D}[\{p^{d}_{j}\}_{p,j}](k_1,k_2,-k_3) \;,
\end{aligned}
\end{equation}
where $H_{2D}[\{p^{0}_{j}\}_{p,j}](k_1,k_2,0)$ is the tight-binding model limited to the basal plane. 


\section{Systematic 3D embedding of 2D models}\label{3D_embedding}

In the three-dimensional Brillouin zone $k_3 = 0$ and $k_3=1$ define the two $C_2\mathcal{T}$ symmetric planes. The non-Abelian braiding of Weyl points happens within these planes. For clarity we isolate the braiding protocol to the plane $k_3=0$ by requiring that all the  $(k_1,k_2)$-dependent terms vanish at $k_3=1$ which guarantees that the band structure is featureless there, while the terms that do not depend on $(k_1,k_2)$ will be used to control the band gaps at $k_3=0$ and $k_3=1$ independently (see below). It is now straightforward from Eq.~(\ref{eq_generic_3D}) to define the conditions that realize this. Indeed, from 
\begin{equation*}
\begin{aligned}
    H_{3D}[\{p^{0,u,d}_{j}\}_{p,j}](k_1,k_2,1) &= H_{2D}[\{p^{0}_{j}\}_{p,j}](k_1,k_2,0) \\ &+ H_{2D}[\{p^{u}_{j}\}_{p,j}](k_1,k_2,1) \\
    &+ H_{2D}[\{p^{d}_{j}\}_{p,j}](k_1,k_2,1)\;,\\
    &= H_{2D}[\{p^{0}_{j}\}_{p,j}](k_1,k_2,0) \\
    &- H_{2D}[\{p^{u}_{j}\}_{p,j}](k_1,k_2,0) \\
    &- H_{2D}[\{p^{d}_{j}\}_{p,j}](k_1,k_2,0)\;, 
\end{aligned}
\end{equation*}
we have that $H_{3D}[\{p^{0,u,d}_{j}\}_{p,j\neq0}](k_1,k_2,1) = 0$ is readily satisfied if $p^{0}_{j}-p^{u}_{j}-p^{d}_{j} = 0$ for $j\neq0$. 

For instance for $p=a$ we get $a^0_j - a^u_j - a^d_j = 0$. But since $a^d_j = a^u_j$, it reduces to $a^u_j = a^0_j/2$. For $p=b$ we first get $b^0_j - b^u_j - b^d_j = 0$. In principle, the phases of the $b^{0,u,d}_j$'s are free to differ, however, for simplicity we take them equal without significant loss of generality. Then, by setting $b^d_j = \beta_j b^0_j$ (with $\beta_j$ real), the constraint is satisfied for $b^u_j = (1-\beta_j) b^0_j $.  

Collecting all the conditions together, these are 
\begin{equation}
\begin{array}{ll}
	a^{u}_j = a^0_j/2 \;, & \\ 
	b^{u}_j = (1-\beta_j)b^0_j  \;, & b^{d}_j = \beta_j b^0_j\;, 
\end{array}
\end{equation}
for $j=1,\dots,4$ and where $\beta_j \in [0,1]$ are free parameters, and 
\begin{equation}
\begin{array}{ll}
	d^{u}_j = (1-\delta_j)d^0_j  \;, & d^{d}_j = \delta_j d^0_j/2\;,  \\ 
	f^{u}_j = f^0_j \;, & \\ 
\end{array}
\end{equation}
for $j=1,\dots,8$ and where $\delta_j \in [0,1]$ is an other free parameter. %he factor $1/2$ comes from the fact that we cancel a $p^{u}_{j}$- and a $p^{d}_{j}$-term with a single $p^{0}_{j}$-term.  

As for the $(k_1,k_2)$-independent terms, we impose the same constraint of cancellation at $k_3=1$ for $a^{0,u}_0$, $b^{0,u}_0$, and $f^{0,u}_0$, while we impose the cancellation condition at $k_3=0$ for $d^{0,u,d}_0$. This allows us to control the gaps between the bands at $k_3=0$ and at $k_3=1$ independently. That gives, 
\begin{equation}
\begin{array}{ll}
	a^u_0 = a^0_0/2 \,,& b^u_0 = b^0_0/2 \,,\\
	f^u_0 = f^0_0/2 \,,& \\
	d^u_0 = -(1-\delta_0) d_0^0 \,, & d^d_0 = -\delta_0 d_0^0 \;.
\end{array}
\end{equation} 
Note the minus signs for the $d^{0,u,d}_0$'s. 


\subsection{Free parameters for the braiding protocol} 

We list the remaining free parameters by which the protocol of the three-dimensional braiding of Weyl nodes is defined. The free complex variables are $\{a^0_j,b^0_j\}_{j=1,\dots,4}$, $\{d^0_j,f^0_j\}_{j=1,\dots,8}$, and $\{d_0^0,f_0^0\}$. The free real variables are $\{a^0_0,b^0_0\}$, $\{\beta_j\}_{j=1,\dots,4}$, $\{\delta_j\}_{j=1,\dots,8}$, and $\delta_0$. 

Importantly, we also uncover three-dimensional generalizations, and discuss possible experimental realizations in van-der-Waals heterostructures.

In Fig.~\ref{fig:braiding3D}{\bf c--d} we illustrate the four scenarios using data obtained from explicit 3D tight-binding models, detailed in the Supplemental Material~\cite{Supp}.
The trajectories of the principal WPs (solid opaque lines) and adjacent WPs (ragged transparent lines) are marked according to their chirality (green vs.~magenta) and are given a time direction through the arrows. The spheres indicate the position of the WPs at the end of the protocol. In both cases we assume that two adjacent WPs are first created within the symmetric plane [({\bf E}) in Fig.~\ref{fig:braiding3D}{\bf c}, and ({\bf C}) in Fig.~\ref{fig:braiding3D}{\bf d}], which are then driven through a non-contractible loop in the Brillouin zone, each WP in opposite direction, until they disappear by colliding at the end of their trajectories within the plane [({\bf A}) in Fig.~\ref{fig:braiding3D}{\bf c}, and ({\bf C}) in Fig.~\ref{fig:braiding3D}{\bf d}]. Then follows the creation of two principal WPs within the symmetric plane [({\bf C}) in Fig.~\ref{fig:braiding3D}{\bf c}, and ({\bf E}) in Fig.~\ref{fig:braiding3D}{\bf d}], that are sent in opposite directions over a non-contractible path in the Brillouin zone that crosses the past trajectory of the adjacent WPs. This induces a nontrivial frame-rotation charge upon the principal WPs at the end of their trajectories, such that these experience an obstruction to leave the plane [({\bf D}) in Fig.~\ref{fig:braiding3D}{\bf c}, and ({\bf B}) in Fig.~\ref{fig:braiding3D}{\bf d}].



\section{Conversion by braiding analysis in 3D}
We present here the numerical data and discuss the scenarios when two principal WPs collide within a $C_2\mathcal{T}$ symmetric plane depending on their braiding with adjacent WPs. We organize the braiding protocol such that the obstruction to leave the symmetric plane happens for the principal WPs. 

\subsubsection{WP location within the symmetric plane}

In Fig.~\ref{fig:protocol_3D_data} we draw the product of the magnitude of the two gaps, principal and adjacent, over the 2D Brillouin zone at the symmetric plane $k_3=0$. Lighter (darker orange) color indicates larger (smaller) gaps (principal and adjacent combined). The dark spots indicate the location of WPs. 

Fig.~\ref{fig:protocol_3D_data}{\bf a} ({\bf b}) corresponds to the process of Fig.~5{\bf c} (respectively, {\bf d}) of the main text. Following the main text, we label the processes between two WPs that meet as ({\bf A}), ({\bf B}), ({\bf C}), ({\bf D}), and ({\bf E}), see below and in Fig.~5 of the main text.   

In Fig.~\ref{fig:protocol_3D_data}{\bf a} we start (panel~1) with the creation of two secondary WPs of equal chirality within the symmetric plane ({\bf E}). Then we collide them after they run, each in opposite direction, through a non-contractible loop of the Brillouin zone (panels~2--3). Since there has been no braiding for them, they can leave the plane, one above and one below ({\bf A}). A pair of principal WPs of opposite chirality is now created ({\bf C}) (panel~4). We make them collide after they run, each in opposite direction, along a non-contractible loop that crosses the past trajectory of the adjacent WPs (panels~5--7). Due to the nontrivial frame-rotation charge they acquired through the braiding with the adjacent WPs, these do not annihilate and bounce back within the symmetric plane ({\bf D}) (panel~8). 


In Fig.~\ref{fig:protocol_3D_data}{\bf b} we start (panel~1) with the creation of two principal WPs of equal chirality within the symmetric plane ({\bf E}). Two adjacent WPs of opposite chirality are then created ({\bf C}) (panel~2). We collide the adjacent WPs after they run, each in opposite direction, through a non-contractible loop of the Brillouin zone (panels~3--4). Since there has been no braiding for them, they can leave the plane through annihilation ({\bf C}). We then collide the principal WPs after they run, each in opposite direction, through a non-contractible loop (panels~5--6). Since their trajectory crosses the past trajectory of the adjacent WPs they acquired a nontrivial frame-rotation charge which forbids them to leave the symmetric plane, so that they bounce away within the plane ({\bf B}) (panel~7). 

\subsubsection{Values of the tight-binding parameters}

The tight-binding parameters for the protocol of Fig.~\ref{fig:protocol_3D_data}{\bf a}, and  Fig.~\ref{fig:protocol_3D_data}{\bf b}, are given in Table \ref{TB_table_I}~A, and Table \ref{TB_table_I}~B, respectively. The tight-binding parameters of Table \ref{TB_table_I} are themselves defined in terms of control parameters which values determine the WP configuration at a given ``time'' of the protocol. We list the values of the control parameters corresponding to the snapshots of Fig.~\ref{fig:protocol_3D_data}{\bf a}, and  Fig.~\ref{fig:protocol_3D_data}{\bf b}, in Table \ref{TB_table_II}~A, and Table \ref{TB_table_II}~B, respectively. 



\subsubsection{Chirality of each pair of WPs}

The identification of the processes ({\bf A}, {\bf B}, {\bf C}, {\bf D}, {\bf E}) requires the computation of the chiral charge of the WP pair involved. We show in Fig.~\ref{fig:chirality_3D} the in-plane band structure with a pair of WPs (left column) and the computation of the corresponding chirality (right column) at snapshots of the 3D braiding protocol Fig.~\ref{fig:protocol_3D_data}. The chirality is obtained as the winding number of the flow of Berry phase as we sweep a base loop over a sphere wrapping the WP pair from a north pole (NP) above the symmetry plane to a south pole (SP) underneath the symmetric plane, and with the equator (E) defining a loop within the symmetric plane (visible as the black line on the left column). 

Fig.~\ref{fig:chirality_3D}{\bf a} captures the adjacent WP pair between ({\bf E}) and ({\bf A}) of Fig.~\ref{fig:protocol_3D_data}{\bf a}, giving a chirality of $+2$, i.e. the WPs have equal chirality. Fig.~\ref{fig:chirality_3D}{\bf b} captures the principal WP pair between ({\bf C}) and ({\bf D}) of Fig.~\ref{fig:protocol_3D_data}{\bf a}, revealing that these have opposite chirality (since the total chirality is zero). 

Fig.~\ref{fig:chirality_3D}{\bf c} captures the adjacent WP pair between ({\bf C}) and ({\bf C}) of Fig.~\ref{fig:protocol_3D_data}{\bf b}, revealing that they have an opposite chirality. Fig.~\ref{fig:chirality_3D}{\bf d} captures the principal WP pair between ({\bf E}) and ({\bf B}) of Fig.~\ref{fig:protocol_3D_data}{\bf b}, revealing that these have equal chirality.
 
\subsubsection{Stable critical points} 
 
Finally, we show in Fig.~\ref{fig:critical_points_3D}{\bf a}, and {\bf b}, the band structures at the stable critical points of Fig.~\ref{fig:protocol_3D_data}{\bf a}, and Fig.~\ref{fig:protocol_3D_data}{\bf b} respectively, i.e. when the two principal WPs meet exactly before to bounce away through the process ({\bf D}), and ({\bf B}) respectively. The band structure shows a two-dimensional slice of the 3D band structures with one direction taken within the symmetric plane and the other direction taken along the vertical axis $(001)$ for $k_3\in[0,1]$. 







%%%%%%%%%%%%%%%%%%%% FIGURE HERE %%%%%%%%%%%%%%%%%%%%
\begin{figure*}[htpb!]
\centering
\begin{tabular}{l}
{\bf a} \\
\begin{tabular}{llll} 
	1.\includegraphics[width=0.22\linewidth]{figs/3D_braiding_c_1.pdf} &
	2.\includegraphics[width=0.22\linewidth]{figs/3D_braiding_c_2.pdf} &
	3.\includegraphics[width=0.22\linewidth]{figs/3D_braiding_c_3.pdf} &
	4.\includegraphics[width=0.22\linewidth]{figs/3D_braiding_c_4.pdf} \\
	5.\includegraphics[width=0.22\linewidth]{figs/3D_braiding_c_5.pdf} &
	6.\includegraphics[width=0.22\linewidth]{figs/3D_braiding_c_6.pdf} &
	7.\includegraphics[width=0.22\linewidth]{figs/3D_braiding_c_7.pdf} &
	8.\includegraphics[width=0.22\linewidth]{figs/3D_braiding_c_8.pdf} 
\end{tabular}\\
{\bf b}\\
\begin{tabular}{llll} 
	1.\includegraphics[width=0.22\linewidth]{figs/3D_braiding_d_1.pdf} &
	2.\includegraphics[width=0.22\linewidth]{figs/3D_braiding_d_2.pdf} &
	3.\includegraphics[width=0.22\linewidth]{figs/3D_braiding_d_3.pdf} &
	4.\includegraphics[width=0.22\linewidth]{figs/3D_braiding_d_4.pdf} \\
	5.\includegraphics[width=0.22\linewidth]{figs/3D_braiding_d_5.pdf} &
	6.\includegraphics[width=0.22\linewidth]{figs/3D_braiding_d_6.pdf} &
	7.\includegraphics[width=0.22\linewidth]{figs/3D_braiding_d_7.pdf} &
\end{tabular}\\
\end{tabular}\\
\caption{\textsf{\textbf{3D braiding protocol.} Product of the magnitude of the two gaps, principal and adjacent, over the 2D Brillouin zone at the symmetric plane $k_3=0$. Lighter (darker orange) color indicates larger (smaller) gaps (principal and adjacent combined). The dark spots indicate the location of WPs. {\bf a} Numerical data corresponding to the process of Fig.~5{\bf c} of the main text with the successive steps ({\bf E}), and ({\bf A}) for the adjacent WPs, and then ({\bf C}), and ({\bf D}) for the principal WPs. {\bf b} Numerical data corresponding to the process of Fig.~5{\bf d} of the main text with the successive steps ({\bf E}) for principal WPs, ({\bf C}) for adjacent WPs, and again ({\bf C}) for adjacent WPs, and eventually ({\bf B}) for principal WPs.}}
\label{fig:protocol_3D_data} 
\end{figure*}
%%%%%%%%%%%%%%%%%%%% FIGURE HERE %%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%% FIGURE HERE %%%%%%%%%%%%%%%%%%%%
\begin{figure}[htpb!]
\centering
\begin{tabular}{ll}
{\bf a} & \\
	\includegraphics[width=0.55\linewidth]{figs/chirality_c_E_A_BS.pdf} & 
	\includegraphics[width=0.45\linewidth]{figs/chirality_c_E_A.pdf} \\
	{\bf b} & \\
	\includegraphics[width=0.55\linewidth]{figs/chirality_c_C_D_BS.pdf} & 
	\includegraphics[width=0.45\linewidth]{figs/chirality_c_C_D.pdf} \\
{\bf c} & \\
		\includegraphics[width=0.55\linewidth]{figs/chirality_d_C_C_BS.pdf} & 
	\includegraphics[width=0.45\linewidth]{figs/chirality_d_C_C.pdf} \\
	{\bf d} &  \\
	\includegraphics[width=0.55\linewidth]{figs/chirality_d_E_B_BS.pdf} & 
	\includegraphics[width=0.45\linewidth]{figs/chirality_d_E_B.pdf} 
\end{tabular} 
\caption{\textsf{\textbf{Weyl point pair chirality.} Left column: Band structure within the symmetric plane with the pairs of Weyl points (WPs) involved in the processes ({\bf A}), ({\bf B}), ({\bf C}), ({\bf D}), and ({\bf E}) of Fig.~\ref{fig:protocol_3D_data}. Right column: Flow of Berry phase over a base sphere, wrapping each pair of WPs, from the north pole (NP), above the symmetric plane, to the south pole (SP), underneath the plane, and with the equator (E) intersecting the plane (black circle in the figures on the left). {\bf a} WP pair between ({\bf E}) and ({\bf A}) of Fig.~\ref{fig:protocol_3D_data}{\bf a}. {\bf b} WP pair between ({\bf C}) and ({\bf D}) of Fig.~\ref{fig:protocol_3D_data}{\bf a}. {\bf c} WP pair between ({\bf C}) and ({\bf C}) of Fig.~\ref{fig:protocol_3D_data}{\bf b}. {\bf d} WP pair between ({\bf E}) and ({\bf B}) of Fig.~\ref{fig:protocol_3D_data}{\bf b}.}}
\label{fig:chirality_3D} 
\end{figure}
%%%%%%%%%%%%%%%%%%%% FIGURE HERE %%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%% FIGURE HERE %%%%%%%%%%%%%%%%%%%%
\begin{figure}[htpb!]
\centering
\begin{tabular}{l}
{\bf a}\\
	\includegraphics[width=0.6\linewidth]{figs/3D_braiding_c_BS.pdf} \\
	{\bf b}\\
	\includegraphics[width=0.6\linewidth]{figs/3D_braiding_d_BS.png} 
\end{tabular}
\caption{\textsf{\textbf{Stable critical points of the 3D braiding protocol.} {\bf a} Band structure at $k_1=0.13\pi$ for $(k_2,k_3)\in [-1,1]\times [0,1]$ at the critical point ({\bf D}) of the braiding protocol Fig.~\ref{fig:protocol_3D_data}{\bf a}. {\bf b} Band structure at $k_2=0.31\pi$ for $(k_1,k_3)\in [-1,1]\times [0,1]$ at the critical point ({\bf B}) of the braiding protocol Fig.~\ref{fig:protocol_3D_data}{\bf b}. }}
\label{fig:critical_points_3D} 
\end{figure}
%%%%%%%%%%%%%%%%%%%% FIGURE HERE %%%%%%%%%%%%%%%%%%%%

 
\begin{table*}[htpb!]
\centering
\caption{\textsf{\label{TB_table_I} Tight-binding parameters for the 3D braiding protocol of Fig.~\ref{fig:protocol_3D_data} parameterized as functions of the control parameters $\{p_0,p_1,p_2,p_3,p_4,p_5,p_6\}$, see Table \ref{TB_table_II}. \vspace{0.5cm}
}}
%\begin{tabular*}{\linewidth}{c @{\extracolsep{\fill}} c c }
\begin{tabular}{l}
A.~Tight-binding parameters for Fig.~\ref{fig:protocol_3D_data}{\bf a}. \\
\begin{tabular}{lll}
\hline \\
$a^0_0 = 0.5 p_0 $ & 
	$b^u_0 = 0$ &
		$ f^0_0 = 0.85 e^{-i 0.1 \pi}$ \\
$a^0_1 = i(0.45 p_3 + 0.045 p_4) $ & 
	$ d^0_0 = 3.33  $ &
		$ f^0_1 = i ( p_1  + 0.35 p_3) e^{i 0.2 \pi }$ \\
$a^0_2 = -0.3 p_3 $ & 
	$ d^0_1 = -0.1 p_3$ &
		$ f^0_2 = (-0.125 p_1  - 0.3 p_3 - 0.05 p_4) e^{i 0.2 \pi}$ \\
$a^0_3 = -0.2 p_3 $ & 
	$d^0_2 = 0.2  e^{i  0.1 \pi} p_3 $ &
		$ f^0_3 =( 0.5 p_1 - 0.03 p_4) e^{i 0.2 \pi }$ \\
$a^0_4 = 0.1 p_3 $ & 
	$d^0_3 = (0.2 p_3 + 0.029 p_4 ) e^{-i 0.099 \pi} $ &
		$ f^0_4 = -0.25 p_3 $ \\
$b^0_0 = 0$ & 
	$d^0_4 = -0.2  e^{-i 0.2 \pi} p_3$ &
		$ f^0_5 = 0.55  p_3 - 0.7 p_5 $  \\
$b^0_1 =0$ & 
	$d^0_5 = 0.333 e^{-i 0.45 \pi} p_2 $ & 
		$ f^0_6 =  0 $  \\
$b^0_2 =-0.03 p_4$ & 
	$d^0_6 = 0 $ &
		$ f^0_7 = 0 $ \\
$b^0_3 =0$ &   
	$d^0_7 = i 0.667   e^{- i 0.45 \pi} p_2 $ &
		 $ f^0_8 =  0.5 p_3 + 0.05 p_4 $ \\
$b^0_4 =-0.1 p_3$ & 
	$d^0_8 = -0.05  e^{-i 0.2 \pi } p_3 $ &  $a^u_0 = 0.25 p_0$
%\end{tabular*}
\end{tabular} \\
\\
B.~Tight-binding parameters for Fig.~\ref{fig:protocol_3D_data}{\bf b}. \\
\hline \\
\begin{tabular}{lll}
$a^0_0 = 4.5 - 3.5 p_3$ & 
	$b^u_0 = 0$ &
		$ f^0_0 = 1.25 $ \\
$a^0_1 = 0 $ & 
	$ d^0_0 = 2.67 e^{- i 0.35 \pi} $ &
		$ f^0_1 = i ( 0.5 p_1 - 0.1 p_4 ) e^{-i 0.15 \pi} $ \\
$a^0_2 = 0 $ & 
	$ d^0_1 = -1.333 p_4 $ &
		$ f^0_2 = 0.125 p_1  $ \\
$a^0_3 = - p_4 $ & 
	$d^0_2 = -0.1667 p_4 $ &
		$ f^0_3 = (0.5 p_1 - 0.45 p_4 ) e^{-i 0.15 \pi}$ \\
$a^0_4 = 0.35 p_4 $ & 
	$d^0_3 = ( -0.1667 p_2 - 0.2667 p_4 + 0.0005 p_5 e^{-i  0.0015 \pi} ) $ &
		$ f^0_4 = -0.55 p_3 $ \\
$b^0_0 = 0$ & 
	$d^0_4 = 0.1667 p_4 $ &
		$ f^0_5 = -0.5 p_3 - 0.001667 p_5 $  \\
$b^0_1 = -0.5 p_3$ & 
	$d^0_5 = ( 0.333 p_2  - 0.000333 p_5 ) e^{i 0.2 \pi}$ & 
		$ f^0_6 =  -0.3 p_3 $  \\
$b^0_2 =0$ & 
	$d^0_6 = 0.1 p_5 e^{-i 0.06 \pi} $ &
		$ f^0_7 = 0.55 p_4 $ \\
$b^0_3 = 0.5 p_4 $ &   
	$d^0_7 = i ( 0.667 p_2 + 0.0667 p_5) e^{i 0.2 \pi} $ &
		 $ f^0_8 =  0.3 p_3 $ \\
$b^0_4 = 0.5 p_4 $ & 
	$d^0_8 = 0.333 p_6 $ & $a^u_0 = 2.25 - 1.75 p_3$
%\end{tabular*}
\end{tabular}
\end{tabular}
\end{table*} 


\begin{table*}[htpb!]
\centering
\caption{\textsf{\label{TB_table_II} Values of the control parameters $\{p_0,p_1,p_2,p_3,p_4,p_5,p_6\}$ entering Table \ref{TB_table_I} and corresponding to the snapshots of Fig.~\ref{fig:protocol_3D_data}. \vspace{0.5cm}
}}
%\begin{tabular*}{\linewidth}{c @{\extracolsep{\fill}} c c }
%\end{tabular*}
\begin{tabular}{l}
A.~Control parameters for the snapshots of Fig.~\ref{fig:protocol_3D_data}{\bf a}.  \\
\begin{tabular}{l | llllll}
\hline 
1.& $p_0 = 10.4 $ & 
	$p_1 = 0.6 $ &
		$p_2 = 1 $ &
			$p_3 = 0 $ & 
				$ p_4 = 0 $ &
					$ p_5 = 0 $ \\
2.& $p_0 = 10.4 $ & 
	$p_1 = 1 $ &
		$p_2 = 1 $ &
			$p_3 = 0 $ & 
				$ p_4 = 0 $ &
					$ p_5 = 0 $ \\
3.& $p_0 = 10.4 $ & 
	$p_1 =  1.4 $ &
		$p_2 = 1 $ &
			$p_3 = 0 $ & 
				$ p_4 = 0 $ &
					$ p_5 = 0 $ \\
4.& $p_0 = 6.76 $ & 
	$p_1 =  2 $ &
		$p_2 = 1 $ &
			$p_3 = 0 $ & 
				$ p_4 = 0 $ &
					$ p_5 = 0 $ \\
5.& $p_0 = 5.2 $ & 
	$p_1 =  2 $ &
		$p_2 = 1 $ &
			$p_3 = 0 $ & 
				$ p_4 = 0 $ &
					$ p_5 = 0 $ \\
6.& $p_0 = 5.2 $ & 
	$p_1 =  2 $ &
		$p_2 = 1 $ &
			$p_3 = 1 $ & 
				$ p_4 = 0 $ &
					$ p_5 = 0 $ \\
7.& $p_0 = 5.2 $ & 
	$p_1 =  2 $ &
		$p_2 = 1 $ &
			$p_3 = 1 $ & 
				$ p_4 = 1 $ &
					$ p_5 = 0 $ \\
8.& $p_0 = 5.2 $ & 
	$p_1 =  2 $ &
		$p_2 = 1 $ &
			$p_3 = 1 $ & 
				$ p_4 = 1 $ &
					$ p_5 = 1 $ 
\end{tabular} \\
\\
B.~Control parameters for the snapshots of Fig.~\ref{fig:protocol_3D_data}{\bf b}. \\
\hline 
\begin{tabular}{l | llllll}
1.& $p_1 = 1.6  $ & 
	$p_2 =  1 $ &
		$p_3 = 0 $ &
			$p_4 = 0 $ & 
				$ p_5 = 0 $ &
					$ p_6 = 0 $ \\
2.& $p_1 = 2.48 $ & 
	$p_2 =  1.24 $ &
		$p_3 = 0.3 $ &
			$p_4 = 0 $ & 
				$ p_5 = 0 $ &
					$ p_6 = 0 $ \\
3.& $p_1 = 2.8 $ & 
	$p_2 =  1.4 $ &
		$p_3 = 0.5 $ &
			$p_4 = 0 $ & 
				$ p_5 = 0 $ &
					$ p_6 = 0 $ \\
4.& $p_1 = 3.12 $ & 
	$p_2 =  1.56 $ &
		$p_3 = 0.7 $ &
			$p_4 = 0 $ & 
				$ p_5 = 0 $ &
					$ p_6 = 0 $ \\
5.& $p_1 = 3.6 $ & 
	$p_2 =  1.8 $ &
		$p_3 = 1 $ &
			$p_4 = 0.5 $ & 
				$ p_5 = 0 $ &
					$ p_6 = 0 $ \\
6.& $p_1 = 3.6 $ & 
	$p_2 =  1.8 $ &
		$p_3 = 1 $ &
			$p_4 = 1 $ & 
				$ p_5 = 1 $ &
					$ p_6 = 0 $ \\
7.& $p_1 = 3.6 $ & 
	$p_2 =  1.8 $ &
		$p_3 = 1 $ &
			$p_4 = 1 $ & 
				$ p_5 = 1 $ &
					$ p_6 = 1 $ 
%\end{tabular*}
\end{tabular}
\end{tabular}
\end{table*}            
  
  
  
\appendix


\section{Extra relations}

Let us write $\hat{h}_{ij}$ the symmetric matrix with the single non-zero elements, $[\hat{h}_{ij}]_{kl}  = \delta_{ik}\delta_{jl} + \delta_{il}\delta_{jk} = [\hat{h}_{ji}]_{kl} $ if $i\neq j$, and $[\hat{h}_{ii}]_{kl}  = \delta_{ik} \delta_{il}$. The conversion from the $\hat{h}$'s matrices to the gamma matrices then reads
\begin{equation}
    \begin{aligned}
        \gamma_{00} &= \dfrac{1}{4} \left( \hat{h}_{11} + \hat{h}_{22} +  \hat{h}_{33} +\hat{h}_{44} \right),\\
        \gamma_{01} &= \dfrac{1}{4} \left( \hat{h}_{12} + \hat{h}_{34} \right),\\
        \gamma_{03} &= \dfrac{1}{4} \left( \hat{h}_{11} - \hat{h}_{22} +  \hat{h}_{33} - \hat{h}_{44} \right),\\
        \gamma_{10} &= \dfrac{1}{4} \left( \hat{h}_{13} + \hat{h}_{24}  \right),\\
        \gamma_{30} &= \dfrac{1}{4} \left( \hat{h}_{11} + \hat{h}_{22} -  \hat{h}_{33} - \hat{h}_{44} \right),\\
        \gamma_{11} &= \dfrac{1}{4} \left( \hat{h}_{14} + \hat{h}_{23} \right),\\
        \gamma_{13} &= \dfrac{1}{4} \left( \hat{h}_{13} - \hat{h}_{24}  \right),\\
        \gamma_{22} &= \dfrac{1}{4} \left(  -\hat{h}_{14} + \hat{h}_{23}   \right),\\
        \gamma_{31} &= \dfrac{1}{4} \left(\hat{h}_{12} - \hat{h}_{34} \right),\\
        \gamma_{33} &= \dfrac{1}{4} \left( \hat{h}_{11} - \hat{h}_{22} -\hat{h}_{33} +\hat{h}_{44}  \right).
    \end{aligned}
\end{equation}


\subsection{UNUSED FIGURE!!!}
%%%%%%%%%%%%%%%%%%%% FIGURE HERE %%%%%%%%%%%%%%%%%%%%
\begin{figure*}[htpb!]
\centering
\begin{tabular}{llll} 
1. & 2. & 3. & 4.\\
	\includegraphics[width=0.22\linewidth]{4B_11/t_0110.pdf} &
	\includegraphics[width=0.22\linewidth]{4B_11/t_0151.pdf} &
	\includegraphics[width=0.22\linewidth]{4B_11/t_0160.pdf} &
	\includegraphics[width=0.22\linewidth]{4B_11/t_0198.pdf} \\
5. & 6. & 7. & 8.\\
	\includegraphics[width=0.22\linewidth]{4B_11/t_0211.pdf} &
	\includegraphics[width=0.22\linewidth]{4B_11/t_0500.pdf} &
	\includegraphics[width=0.22\linewidth]{4B_11/t_0610.pdf} &
	\includegraphics[width=0.22\linewidth]{4B_11/t_0701.pdf} 
\end{tabular}
\caption{\textsf{\textbf{4-band $\vec{\chi} = (1,1)$.} Debraiding  }}
\label{fig:4B_11_debraiding} 
\end{figure*}
%%%%%%%%%%%%%%%%%%%% FIGURE HERE %%%%%%%%%%%%%%%%%%%%



==> Braiding folllow-up/3D_embedding_braiding.tex <==






\section{Review of 2D case}
We first start by shortly reviewing the two dimensional case. As we pointed out in Ref.~\cite{bouhon2019nonabelian}, \textcolor{orange}{discuss also spinless $C_2$.}


\subsection{Minimal 2D model}
\textcolor{orange}{Copied from appendix of present paper!!!!!!!!!!!!!!!!!!!!!!!!}
The minimal 2D tight-binding model presented in Methods realizes the centered orthorhombic layer group $c222$ (LG$22$), with point group $D_2 = \{C_{2z},C_{2y},C_{2x}\}$~\cite{ITCE}. There are three orbitals per unit cell, one $s$-wave orbital at Wyckoff position $1a$ ($\phi_A$) and one (real) $p_z$-wave orbital at Wyckoff position $2g$ ($\phi_B,\phi_C$), see Fig.~\ref{fig:2D_minimal_lattice} where the primitive cell is spanned by the Bravais lattice vectors $\boldsymbol{a}_1 = (a \hat{x} + b \hat{y})/2$ and $\boldsymbol{a}_2 = (-a \hat{x} + b \hat{y})/2$.

% %%%%%%%%%%%%%%%%%%%% FIGURE HERE %%%%%%%%%%%%%%%%%%%%
% \begin{figure}[h]
% \centering
% \includegraphics[width=0.9\linewidth]{figs/minimal_lattice.pdf}
% \caption{\textsf{Crystal structure of the minimal 2D tight-binding model discussed in the main text and presented in Methods. The conventional unit cell (centered orthorhombic) is spanned by $a \hat{x}$ and $b\hat{y}$. There are three orbitals per each primitive cell spanned by the primitive vectors $\boldsymbol{a}_1$ and $\boldsymbol{a}_2$, one s-wave orbital labeled $\phi_A$ (blue), and two $p_z$-wave orbitals labeled $\phi_B$ and $\phi_C$ (green). The point group is $D_2 = \{C_{2z},C_{2(11)}\equiv C_{2y},C_{2(1\bar{1})}\equiv C_{2x}\}$ with $C_{2z}$ perpendicular to the basal plane.}}
% \label{fig:2D_minimal_lattice} 
% \end{figure}
% %%%%%%%%%%%%%%%%%%%% FIGURE HERE %%%%%%%%%%%%%%%%%%%%
% minimal_model_parameters.pdf
 
 



The locations of the orbitals within the $n$-th unit cell are $\{\boldsymbol{R}_n+\boldsymbol{r}_{\alpha}\}_{\alpha=A,B,C}$, with $\boldsymbol{r}_A = (0,0)$ for $1a$, and $\boldsymbol{r}_B = (0,u)$ and $\boldsymbol{r}_C = (0,-u)$ for $2g$ (written in the Cartesian frame) with $u<b/2$. The tight-binding model is written in the Bloch state basis 
\begin{equation}
    \vert \phi_{\alpha} , \boldsymbol{k} \rangle = \dfrac{1}{\sqrt{N_{\alpha}}} \sum_{\boldsymbol{R}_n} e^{\imi \boldsymbol{k} \cdot \boldsymbol{R}_n }\vert w , \boldsymbol{R}_n + \boldsymbol{r}_{\alpha} \rangle \,, \;\alpha=A,B,C\,,
\end{equation}
that is the discrete Fourier transform of the Wannier states $\vert w , \boldsymbol{R}_n + \boldsymbol{r}_{\alpha} \rangle$ localized at $\boldsymbol{R}_n + \boldsymbol{r}_{\alpha}$, with $N_{\alpha}$ the number of lattice sites occupied by orbital $\alpha$. 

%%%%%%%%%%%%%%%%%%%% FIGURE HERE %%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\includegraphics[width=0.7\linewidth]{figs/minimal_model_parameters.pdf}
\caption{\textsf{Tight-binding parameters of the 2D minimal model as functions of the control parameter $t$. }}
\label{fig:2D_minimal_parameters} 
\end{figure}
%%%%%%%%%%%%%%%%%%%% FIGURE HERE %%%%%%%%%%%%%%%%%%%%
\textcolor{orange}{End Copied from appendix of present paper!!!!!!!!!!!!!!!!!!!!!!!!}

 The 2D minimal model discussed in Ref.~\cite{bouhon2019nonabelian} can be formulated in terms of the generic tight-binding model as follows.  Since the model is defined within a single basal plane only we introduce the following parameters.
 
 \textcolor{orange}{Start with setup}
, we first set $p^{u,d}_j = 0$ for all $j$. Then, among the basal tight-binding terms only the following are set to finite values $\{a^0_0,d^0_5,d^0_7,f^0_0,f^0_1,f^0_3\}$. 


Importantly, the overly simplified form of the minimal model leads to an effective auxiliary $C_2$ symmetry 
\begin{equation}
\label{eq_C2_bis}
    U (1\oplus \sigma_x) H(C_2\boldsymbol{k}) (1\oplus \sigma_x) U^{\dagger}  = H(\boldsymbol{k}) \;,
\end{equation}
with $U=\mathrm{diag}(-1,1,1)$ corresponding to the gauge transformation $\phi_A\rightarrow -\phi_A$. This can be straightforwardly verified from the explicit expressions Eq.~(\ref{eqn:Ham-matrix_sup}) and (\ref{eq_2}). 

As a consequence of this effective symmetry, the band structure is $C_2$ symmetric and Weyl points (WPs) can only be created four at a time, i.e.~two pairs of WPs with opposite chirality. Indeed, any WP at $\boldsymbol{k}$ must have its symmetric partner of equal chirality at $C_2\boldsymbol{k}$, and these must have their symmetric partners of opposite chirality at $-C_2\boldsymbol{k}$ and $-\boldsymbol{k}$ due to $C_2\mathcal{T}$ symmetry. This property is relaxed in the model used for the 3D protocol of the main text, see Section A7. 

\subsection{Braiding and conversion}
Using free parameters we now discuss the braiding.


Introducing the parameter $t$ that controls the braiding and using the notations of the main text, we obtain the minimal model
\begin{equation}
H_{2D}(\bs{k};t) = \left(\begin{array}{ccc}
f(t)       &   g(\bs{k})      &   g^*(\bs{k})    \\
g^*(\bs{k})    &   0              &   h(\bs{k};t)      \\
g(\bs{k})      &   h^*(\bs{k};t)  &   0   
\end{array}\right)\;, \label{eqn:Ham-matrix_sup} %:)
\end{equation}
where 
\begin{equation}
\label{eq_2}
\begin{aligned}
    f(t) &= a^0_0(t) \;, \\
    g(\bs{k}) &= d^0_5 \e{-\imi k_1 \pi} + d^0_7 \e{-\imi k_2\pi} \;,\\
    %=-\imi(\e{-\imi k_1 \pi}-\e{-\imi k_2\pi})\;,\\
    h(\bs{k};t) &= f^0_0(t) + f^0_1(t) \e{\imi k_1 \pi}+ f^0_3(t)  \e{\imi k_2 \pi} \;,
\end{aligned}
\end{equation}
and
\begin{equation}
\label{eq_3}
    \begin{array}{rclrcl}
        a^0_0(t) &=& F_{[8,-]}(t) \,, & f^0_0(t) &=& F_{[2,-]}(t) \\
        d^0_5 &=& -\imi \,, & f^0_1(t) &=& 10-F_{[8,+]}(t) \,, \\
        d^0_7 &=& \imi \,, & f^0_3(t) &=& f^0_1(t) \,,
    \end{array}
\end{equation}
with the $t$-dependent functions defined through $F_{[\rho,\pm]}(t) = 1/2(\vert t+\nu \vert\pm \vert t-\nu \vert)$, see Fig.~\ref{fig:2D_minimal_parameters}. 





\section{Models for non-Abelian reciprocal braiding in 3D}

\subsection{3D embedding of the minimal 2D model}


The minimal 2D model can be readily embedded into 3D using the above insights. In order to have all bands gapped at $k_3=1$, we set the extra parameter $d^0_0 = 4\imi $, while all the other basal parameters are kept the same as in the 2D case. We remark that this preserves the auxiliary $C_2$ symmetry Eq.~(\ref{eq_C2_bis}) so that WPs must be created or annihilated four at a time.  

In Fig.~\ref{fig:protocol_3D_embedded} we show the 3D embedding of the minimal 2D model at successive snapshots for $t\in[-10,10]$. The 3D band structures are represented through two-dimensional slices taken, in one direction, along the diagonals $(1\bar{1}0)$ and $(110)$ (connecting $\Gamma$ to M), and then $(100)$ (connecting $\Gamma$ to X), successively, and, in the other direction, along $(001)$ for $k_3\in[0,1]$, i.e. along the $C_2$ axis perpendicular to the basal plane. 

We start with the three bands gapped ($t=-10$), then four WPs are created in the second gap at $\Gamma$ ($t=-9$), with two WPs of equal chirality moving towards M along the $(1\bar{1}0)$ diagonal and two WPs with the other chirality located outside the symmetric plane, one above and one underneath $\Gamma$ ($t=-8$). Note that by the effective $C_2$ symmetry, the two WPs above and underneath $\Gamma$ are trapped on the $C_2$ axis crossing $\Gamma$.   

At $t=-4$, two WPs of equal chirality have been created in the first gap at M, above and underneath which we find their two partners of creation. The later are again trapped on the $C_2$ axis crossing M, as imposed by the effective $C_2$ symmetry. The two WPs within the symmetric plane ($k_3=0$) are heading along the diagonal $(110)$ towards $\Gamma$, where they meet at the later time $t=-2$. These do not leave the symmetric plane though, as we find them at $t=0$ moving now along the diagonal $(1\bar{1}0)$. 

At $t=2$, the two WPs of the second gap within the symmetric plane meet at M without leaving the plane, as we can see at $t=4$ where they now move along $(110)$ towards $\Gamma$. At $t=8$, they have reached $\Gamma$ where they recombine and annihilate with their two partners of creation. At $t=9$, the WPs of the first gap within the symmetric plane meet eventually at M where they also recombine and annihilate with their two partners of creation.    


As discussed in the main text, the non-Abelian frame-rotation charge captures the stability of two WPs colliding within a $C_2\mathcal{T}$ symmetric plane. On the hand, we have found above (Fig.~\ref{fig:protocol_3D_embedded}) that equal chirality WPs from one gap bounce away as a consequence of the braiding with the WPs of the adjacent gap. On the other hand, we illustrate the case without braiding in Fig.~\ref{fig:protocol_3D_embedded_bis}. In this case, there is no obstruction for two WPs of equal chirality to leave the symmetric plane after colliding, as can be seen in panel 4. of Fig.~\ref{fig:protocol_3D_embedded_bis}. 

%%%%%%%%%%%%%%%%%%%% FIGURE HERE %%%%%%%%%%%%%%%%%%%%
\begin{figure*}[htpb!]
\centering
\begin{tabular}{llll} 
	\includegraphics[width=0.25\linewidth]{figs/3D__BS_6c.png} &
	\includegraphics[width=0.25\linewidth]{figs/3D__BS_6b.png} &
	\includegraphics[width=0.25\linewidth]{figs/3D__BS_6.png} &
	\includegraphics[width=0.25\linewidth]{figs/3D__BS_5.png} \\
	$1.~t=-10$ &
	$2.~t=-9$ &
    $3.~t=-8$ &
	$4.~t=-4$ \\
	\includegraphics[width=0.25\linewidth]{figs/3D__BS_4.png} &
	\includegraphics[width=0.25\linewidth]{figs/3D__BS_34.png} &
	\includegraphics[width=0.25\linewidth]{figs/3D__BS_3.png} &
	\includegraphics[width=0.25\linewidth]{figs/3D__BS_2.png} \\
	$5.~t=-2$ &
	$6.~t=0$ &
	$7.~t=2$ &
	$8.~t=4$ \\
	\includegraphics[width=0.25\linewidth]{figs/3D__BS_1.png} &
	\includegraphics[width=0.25\linewidth]{figs/3D__BS_1c.png} &
	\includegraphics[width=0.25\linewidth]{figs/3D__BS_1b.png} & \\
	$9.~t=8$ &
	$10.~t=9$ &
	$11.~t=10$ & 
\end{tabular}\\
\caption{\textsf{\textbf{3D embedding of the 2D braiding protocol.} The braiding protocol for the minimal 2D model discussed in the main text is controlled by $t$. This setup can be embedded in 3D so that the 2D nodal points are realized as Weyl points within a single $C_2\mathcal{T}$ symmetric plane ($k_3=0$), and with the three bands gapped on the other symmetric plane ($k_3=1$). We draw the two-dimensional slices of the 3D Band structures with the long direction taken as the diagonals $(1\bar{1}0)$ and $(110)$ (connecting $\Gamma$ to M), and $(100)$ (connecting $\Gamma$ to X), and with the second direction taken as $(001)$, i.e. for $k_3\in[0,1]$ (connecting the two $C_2\mathcal{T}$ symmetric planes). }}
\label{fig:protocol_3D_embedded} 
\end{figure*}
%%%%%%%%%%%%%%%%%%%% FIGURE HERE %%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%% FIGURE HERE %%%%%%%%%%%%%%%%%%%%
\begin{figure*}[htpb!]
\centering
\begin{tabular}{llll} 
	\includegraphics[width=0.25\linewidth]{figs/3D__BS_1.png} &
	\includegraphics[width=0.25\linewidth]{figs/3D__BS_7.png} &
	\includegraphics[width=0.25\linewidth]{figs/3D__BS_7b.png} &
	\includegraphics[width=0.25\linewidth]{figs/3D__BS_8.png} \\
	$1.~t=8$ & 2.& 3.&4. 
\end{tabular}\\
\caption{\textsf{\textbf{3D embedding without braiding.} When there is no braiding two WPs of equal chirality are allowed to leave the symmetric plane after colliding. The two WPs of the first gap created at M meet at $\Gamma$ and leave the symmetric plane along the vertical $C_2$ axis. In the middle of the process, we find that the WPs are converted into a nodal line centered on M that crosses the points X and Y of the Brillouin zone, see panel 2. Then in the tird panel the WPs reappeared on $(1\bar{1}0)$, but four extra WPs have emerged out of the nodal line and populate the two vertical $C_2$ axes crossing X and Y (here only X is shown). Eventually, the two WPs within the symmetric plane meet at $\Gamma$ and leave the plane, see panel 4.}}
\label{fig:protocol_3D_embedded_bis} 
\end{figure*}
%%%%%%%%%%%%%%%%%%%% FIGURE HERE %%%%%%%%%%%%%%%%%%%%

\subsection{Generic tight-binding model}
We derive a generic three-dimensional three-band tight-binding model with the single constraint that it satisfies $C_2\mcT$ symmetry with $(C_2\mcT)^2=+1$, and given a choice of the Wyckoff positions. $C_2\mcT$ symmetry requires the magnetic space group $P12'1$ (\#3.3.10) as minimal subgroup \cite{MITC,BradCrack}, i.e. the direct product between the primitive monoclinic Bravais lattice as the normal subgroup of translations and the magnetic point group $2' = \{E,C_2\mcT\}$ (\#3.3.8) with $\hat{y}$ as the $C_2$ rotation axis \cite{MITC,BradCrack}.  

We choose the primitive lattice vectors as $\boldsymbol{a}_1 = a(\sin \theta,0,\cos \theta)$, $\boldsymbol{a}_2 = b(1,0,0)$, and $\boldsymbol{a}_3 = c(0,1,0)$, and write their dual (primitive reciprocal lattice vectors) as $\{\boldsymbol{b}_1,\boldsymbol{b}_2,\boldsymbol{b}_3\}$ ($\boldsymbol{a}_i \cdot \boldsymbol{b}_j = 2\pi \delta_{ij}$) taken as the basis for the Bloch wave vector (momentum) $\boldsymbol{k} = (k_1 \boldsymbol{b}_1+k_2 \boldsymbol{b}_2+k_3 \boldsymbol{b}_3)/2$. Note that the $C_2$ rotation axis ($\hat{y}$ as in \cite{MITC}) is $\boldsymbol{a}_3$ in our basis, i.e.~it acts component-wise on the momentum as $C_2(k_1,k_2,k_3) = (-k_1,-k_2,k_3)$. The $C_2$ rotation axis defines a basal plane perpendicular to it. 

%We note that t
The advantage of the crystallographic convention ($C_2$ taken along $\hat{y}$) is that if we choose $\hat{z}$ as the quantization axis for the spin, the representation of $C^{(\hat{y})}_{2}\mathcal{T}$ symmetry on the pure spinor basis ($\phi_{\uparrow},\phi_{\downarrow}$) takes the simple form $(-\imi\sigma_y)(\imi\sigma_y \mathcal{K}) = \mathbf{1} \mathcal{K}$ (where $\mathcal{K}$ is complex conjugation), i.e.~it makes explicit the fact that it acts trivially on the spin degrees of freedom. As a consequence, our model below holds both for spinful and spinless systems, since it is constrained only by $C_2\mathcal{T}$ symmetry. Form now on we thus discard spin indices and remark explicitly when a statement is only valid for the spinless case.


In the following we make the assumption that one real $s$-wave orbital sits on Wyckoff's positions $1b$ and $2e$ \cite{MITC}. Since $2e$ is twofold ($1b$ is invariant under $C_2$, $2e$ is not) there are three sub-lattice sites per unit cell. We take their locations within the $n$-th unit cell as $\{\boldsymbol{R}_n+\boldsymbol{r}_{\alpha}\}_{\alpha=A,B,C}$, with $\boldsymbol{r}_A = (0,0,0)$ for $1b$, and $\boldsymbol{r}_B = (u,v,w)$ and $\boldsymbol{r}_C = (-u,-v,w)$ for $2e$ (here and in the following we write all vectors of the direct space in the primitive basis $\{\boldsymbol{a}_i\}_{i=1,2,3}$). We write the localized Wannier function for the $\alpha$-th orbital of the $n$-th unit cell as $\vert w , \boldsymbol{R}_n + \boldsymbol{r}_{\alpha} \rangle$. The Bloch basis is then given through the discrete Fourier transform as 
\begin{equation}
    \vert \varphi_{\alpha} , \boldsymbol{k} \rangle = \dfrac{1}{\sqrt{N_{\alpha}}} \sum_{\boldsymbol{R}_n} e^{\imi \boldsymbol{k} \cdot \boldsymbol{R}_n }\vert w , \boldsymbol{R}_n + \boldsymbol{r}_{\alpha} \rangle \,, \;\alpha=A,B,C\,,
\end{equation}%e^{i \boldsymbol{k} \cdot (\boldsymbol{R}_n + \boldsymbol{r}_{\alpha})}
with $N_{\alpha}$ the number of lattice sites with an $\alpha$-orbital. In the following we use the row vector notation $\vert \boldsymbol{\varphi} , \boldsymbol{k} \rangle = \left(\vert \varphi_A , \boldsymbol{k} \rangle ~ \vert \varphi_B , \boldsymbol{k} \rangle ~\vert \varphi_C , \boldsymbol{k} \rangle\right)$. $C_2 \mathcal{T}$ symmetry acts then as
\begin{equation}
    ^{C_2 \mathcal{T}} \vert \boldsymbol{\varphi} , \boldsymbol{k} \rangle = \vert \boldsymbol{\varphi} , (k_1,k_2,-k_3) \rangle (1\oplus \sigma_x) \mathcal{K} \;.
\end{equation}

We can now write the Bloch tight-binding model
\begin{equation}
    \mathcal{H} = \sum_{\boldsymbol{k}\in \mathrm{BZ}} \vert \boldsymbol{\varphi} , \boldsymbol{k} \rangle H(\boldsymbol{k}) \langle \boldsymbol{\varphi} , \boldsymbol{k} \vert\;,
\end{equation}
with the matrix components
\begin{equation}
\label{eq_TB_parameter}
    H_{\alpha\beta}(\boldsymbol{k}) = 
    \sum_{\boldsymbol{n}\in \mathbb{N}^3} 
    T_{\alpha\beta}(\boldsymbol{n}) e^{\imi \boldsymbol{k}\cdot (n_1 \boldsymbol{a}_1+ n_2 \boldsymbol{a}_2 + n_3 \boldsymbol{a}_3 )}\,,
\end{equation}%e^{i \boldsymbol{k}\cdot (\boldsymbol{r}_{\beta}-\boldsymbol{r}_{\alpha} +
where the Bloch wave vector $\boldsymbol{k}= (k_1 \boldsymbol{b}_1+k_2 \boldsymbol{b}_2+k_3 \boldsymbol{b}_3)/2$ is taken within the first Brillouin zone (BZ), i.e. $(k_{1},k_{2},k_{3})\in (-1,1]^{\times 3}$.  


The hopping parameters $T_{\alpha\beta}(\boldsymbol{n}) \in \mathbb{C}$ are constrained by symmetry. First of all, hermiticity imposes 
\begin{equation}
\label{eq_sym_herm}
    T_{\beta\alpha}(\boldsymbol{n}) = T_{\alpha\beta}(-\boldsymbol{n})^*\,.
\end{equation} 
Then, $C_2\mathcal{T}$ requires 
\begin{equation}
    (1\oplus\sigma_x) H^*(k_1,k_2,k_3) (1\oplus\sigma_x) = H(k_1,k_2,-k_3)\;,
\end{equation}
which can be recast into constraints
\begin{equation}
\label{eq_sym_C2T}
\begin{array}{ll}
      T_{AA}(C_2\boldsymbol{n})=T_{AA}(\boldsymbol{n})^* \,,&  
      T_{AC}(C_2\boldsymbol{n})=T_{AB}(\boldsymbol{n})^* \,,\\
      T_{CC}(C_2\boldsymbol{n})=T_{BB}(\boldsymbol{n})^* \,,&
      T_{CB}(C_2\boldsymbol{n})=T_{BC}(\boldsymbol{n})^* \,.
\end{array}
\end{equation}

In the following we choose the parameters $\{T_{BA}(\boldsymbol{n}),T_{BC}(\boldsymbol{n}),T_{CA}(\boldsymbol{n}),T_{AC}(\boldsymbol{n}),T_{CC}(\boldsymbol{n})\}$ as functions of the other parameters, respecting Eqs.~(\ref{eq_sym_herm}) and~(\ref{eq_sym_C2T}). 

\subsection{Explicit 3D model}

Taking the origin $\boldsymbol{0}$ of the Bravais lattice as a reference, and using $\boldsymbol{n}$ of Eq.~(\ref{eq_TB_parameter}) to label its neighbors, we limit the tight-binding model to the following neighbors: from the basal plane $\boldsymbol{n}_0\in \{ (n_1,n_2,0) \in \mathbb{N}^2 \vert n_1, n_2 = -1,0,1\}$, from the first plane above $\boldsymbol{n}_u \in \{ (n_1,n_2,1) \in \mathbb{N}^2 \vert  n_1, n_2 = -1,0,1 \}$, and the first plane below $\boldsymbol{n}_{d} \in \{ (n_1,n_2,-1) \in \mathbb{N}^2 \vert n_1, n_2 = -1,0,1 \}$. In the following we use `$0$', `$u$', and `$d$' to refer respectively to the basal plane, the upper plane (up), and the lower plane (down).

%%%%%%%%%%%%%%%%%%%% FIGURE HERE %%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\includegraphics[width=1.0\linewidth]{figs/FigSup.jpeg}
\caption{\textsf{Schematic representation of the hopping amplitudes. The 3D model is composed of a three atom basis that is arranged in a simple cubic lattice. Considering the site marked by "$0$", in-plane hopping is denoted by $p^{0}_j$, where $j$ refers to the eight neighbors $1-8$. Similarly,  $p^{d}_j$ and $p^{u}_j$ denote hopping to a layer beneath and above, respectively. The specific arrangement of these parameters is outlined in the text. The basis units are colored differently depending on the layer to further elucidate the crystal structure. }}
\label{fig:3D_hopping} 
\end{figure}
%%%%%%%%%%%%%%%%%%%% FIGURE HERE %%%%%%%%%%%%%%%%%%%%

Let us label the neighbors around within each plane clockwise from $1$ to $8$ as a function of $(n_1,n_2)$, i.e.~$1:(1,0)$, $2:(1,1)$, $3:(0,1)$, $4:(-1,1)$, $5:(-1,0)$, $6:(-1,-1)$, $7:(0,-1)$, $8:(1,-1)$, and $0:(0,0)$, see Fig.~\ref{fig:3D_hopping}. We then use a more compact labeling of the parameters as $\{T_{AA}(\boldsymbol{n}_0)\}_{\boldsymbol{n}_0} = \{a^0_{j} \}_{j=0,\dots,8}$, $\{T_{AA}(\boldsymbol{n}_u)\}_{\boldsymbol{n}_u} = \{a^u_{j }\}_{j=0,\dots,8}$, and $\{T_{AA}(\boldsymbol{n}_{d})\}_{\boldsymbol{n}_{d}} = \{a^{d}_{j}\}_{j=0,\dots,8}$. We proceed similarly for $T_{BB} = b $, $T_{CC} = c $, $T_{AB} = d $, $T_{AC} = e $, and $T_{BC} = f $, while the labeling of $T_{BA}$, $T_{BC}$, and $T_{CA}$ is readily given by hermiticity Eq.~(\ref{eq_sym_herm}). 

We can now rewrite the constraints following from Eq.~(\ref{eq_sym_herm}) and (\ref{eq_sym_C2T}) in terms of the compact labeling, i.e.
$$
c^{\mu}_{j+4} = (b^{\mu}_{j })^* ,  \; c^{\mu}_{j} = (b^{\mu}_{j+4 })^* , \; e^{\mu}_{j+4} = (d^{\mu}_{j })^*,  \;e^{\mu}_{j} = (d^{\mu}_{j +4})^*,
$$
for $j=1,\dots,4$ and $\mu=0,u,d$, and $c^{\mu}_{0} = (b^{\mu}_{0})^*$. Note that since the $c$'s and $e$'s are here all determined by the $b$'s and the $d$'s, respectively, we do not refer to them anymore. Then, 
$$a^d_{j} = a^u_{j}\;,\; f^{d}_j = f^{u}_j  \;, $$ 
for $j=0,\dots,8$, and with $a^u_{0} \in \mathbb{R}$. Furthermore, 
$$a^0_{j+4} = (a^0_{j})^*\;,\;b^0_{j+4} = (b^0_{j})^*  \;, $$ 
for $j=1,\dots,4$, and with $a^0_{0},b^0_{0} \in \mathbb{R}$. Finally, 
$$b^d_{j+4} = (b^u_{j})^*\; , \; b^d_{j} = (b^u_{j+4})^*\;,  $$ 
for $j=1,\dots,4$, and $b^d_{0} = (b^u_{0})^*$. In the following, any parameter that is not explicitly constrained to be real is considered as a complex number.



We note that from the form of Eq.~(\ref{eq_TB_parameter}) the three $p^{0,u,d}_{j}$-terms for fixed $p\in\{a,b,d,f\}$ and $j\in\{1,\dots,8\}$ all have the same $(k_1,k_2)$-dependence. On the one hand, the $p^{0}_{j}$-terms have no $k_3$ dependence. On the other hand, the $p^{u}_{j}$- and $p^{d}_{j}$-terms have the form factors of the $p^{0}_{j}$-terms multiplied respectively by $e^{\imi k_3\pi}$, and by $e^{-\imi k_3\pi}$. As a consequence, a generic 3D model has the form
\begin{equation}
\begin{aligned}
\label{eq_generic_3D}
    H_{3D}[\{p^{0,u,d}_{j}\}_{p,j}](k_1,k_2,k_3) &= H_{2D}[\{p^{0}_{j}\}_{p,j}](k_1,k_2,0) \\ 
    &+ H_{2D}[\{p^{u}_{j}\}_{p,j}](k_1,k_2,k_3) \\
    &+H_{2D}[\{p^{d}_{j}\}_{p,j}](k_1,k_2,-k_3) \;,
\end{aligned}
\end{equation}
where $H_{2D}[\{p^{0}_{j}\}_{p,j}](k_1,k_2,0)$ is the tight-binding model limited to the basal plane. 


\section{Systematic 3D embedding of 2D models}\label{3D_embedding}

In the three-dimensional Brillouin zone $k_3 = 0$ and $k_3=1$ define the two $C_2\mathcal{T}$ symmetric planes. The non-Abelian braiding of Weyl points happens within these planes. For clarity we isolate the braiding protocol to the plane $k_3=0$ by requiring that all the  $(k_1,k_2)$-dependent terms vanish at $k_3=1$ which guarantees that the band structure is featureless there, while the terms that do not depend on $(k_1,k_2)$ will be used to control the band gaps at $k_3=0$ and $k_3=1$ independently (see below). It is now straightforward from Eq.~(\ref{eq_generic_3D}) to define the conditions that realize this. Indeed, from 
\begin{equation*}
\begin{aligned}
    H_{3D}[\{p^{0,u,d}_{j}\}_{p,j}](k_1,k_2,1) &= H_{2D}[\{p^{0}_{j}\}_{p,j}](k_1,k_2,0) \\ &+ H_{2D}[\{p^{u}_{j}\}_{p,j}](k_1,k_2,1) \\
    &+ H_{2D}[\{p^{d}_{j}\}_{p,j}](k_1,k_2,1)\;,\\
    &= H_{2D}[\{p^{0}_{j}\}_{p,j}](k_1,k_2,0) \\
    &- H_{2D}[\{p^{u}_{j}\}_{p,j}](k_1,k_2,0) \\
    &- H_{2D}[\{p^{d}_{j}\}_{p,j}](k_1,k_2,0)\;, 
\end{aligned}
\end{equation*}
we have that $H_{3D}[\{p^{0,u,d}_{j}\}_{p,j\neq0}](k_1,k_2,1) = 0$ is readily satisfied if $p^{0}_{j}-p^{u}_{j}-p^{d}_{j} = 0$ for $j\neq0$. 

For instance for $p=a$ we get $a^0_j - a^u_j - a^d_j = 0$. But since $a^d_j = a^u_j$, it reduces to $a^u_j = a^0_j/2$. For $p=b$ we first get $b^0_j - b^u_j - b^d_j = 0$. In principle, the phases of the $b^{0,u,d}_j$'s are free to differ, however, for simplicity we take them equal without significant loss of generality. Then, by setting $b^d_j = \beta_j b^0_j$ (with $\beta_j$ real), the constraint is satisfied for $b^u_j = (1-\beta_j) b^0_j $.  

Collecting all the conditions together, these are 
\begin{equation}
\begin{array}{ll}
	a^{u}_j = a^0_j/2 \;, & \\ 
	b^{u}_j = (1-\beta_j)b^0_j  \;, & b^{d}_j = \beta_j b^0_j\;, 
\end{array}
\end{equation}
for $j=1,\dots,4$ and where $\beta_j \in [0,1]$ are free parameters, and 
\begin{equation}
\begin{array}{ll}
	d^{u}_j = (1-\delta_j)d^0_j  \;, & d^{d}_j = \delta_j d^0_j/2\;,  \\ 
	f^{u}_j = f^0_j \;, & \\ 
\end{array}
\end{equation}
for $j=1,\dots,8$ and where $\delta_j \in [0,1]$ is an other free parameter. %he factor $1/2$ comes from the fact that we cancel a $p^{u}_{j}$- and a $p^{d}_{j}$-term with a single $p^{0}_{j}$-term.  

As for the $(k_1,k_2)$-independent terms, we impose the same constraint of cancellation at $k_3=1$ for $a^{0,u}_0$, $b^{0,u}_0$, and $f^{0,u}_0$, while we impose the cancellation condition at $k_3=0$ for $d^{0,u,d}_0$. This allows us to control the gaps between the bands at $k_3=0$ and at $k_3=1$ independently. That gives, 
\begin{equation}
\begin{array}{ll}
	a^u_0 = a^0_0/2 \,,& b^u_0 = b^0_0/2 \,,\\
	f^u_0 = f^0_0/2 \,,& \\
	d^u_0 = -(1-\delta_0) d_0^0 \,, & d^d_0 = -\delta_0 d_0^0 \;.
\end{array}
\end{equation} 
Note the minus signs for the $d^{0,u,d}_0$'s. 


\subsection{Free parameters for the braiding protocol} 

We list the remaining free parameters by which the protocol of the three-dimensional braiding of Weyl nodes is defined. The free complex variables are $\{a^0_j,b^0_j\}_{j=1,\dots,4}$, $\{d^0_j,f^0_j\}_{j=1,\dots,8}$, and $\{d_0^0,f_0^0\}$. The free real variables are $\{a^0_0,b^0_0\}$, $\{\beta_j\}_{j=1,\dots,4}$, $\{\delta_j\}_{j=1,\dots,8}$, and $\delta_0$. 

Importantly, we also uncover three-dimensional generalizations, and discuss possible experimental realizations in van-der-Waals heterostructures.

In Fig.~\ref{fig:braiding3D}{\bf c--d} we illustrate the four scenarios using data obtained from explicit 3D tight-binding models, detailed in the Supplemental Material~\cite{Supp}.
The trajectories of the principal WPs (solid opaque lines) and adjacent WPs (ragged transparent lines) are marked according to their chirality (green vs.~magenta) and are given a time direction through the arrows. The spheres indicate the position of the WPs at the end of the protocol. In both cases we assume that two adjacent WPs are first created within the symmetric plane [({\bf E}) in Fig.~\ref{fig:braiding3D}{\bf c}, and ({\bf C}) in Fig.~\ref{fig:braiding3D}{\bf d}], which are then driven through a non-contractible loop in the Brillouin zone, each WP in opposite direction, until they disappear by colliding at the end of their trajectories within the plane [({\bf A}) in Fig.~\ref{fig:braiding3D}{\bf c}, and ({\bf C}) in Fig.~\ref{fig:braiding3D}{\bf d}]. Then follows the creation of two principal WPs within the symmetric plane [({\bf C}) in Fig.~\ref{fig:braiding3D}{\bf c}, and ({\bf E}) in Fig.~\ref{fig:braiding3D}{\bf d}], that are sent in opposite directions over a non-contractible path in the Brillouin zone that crosses the past trajectory of the adjacent WPs. This induces a nontrivial frame-rotation charge upon the principal WPs at the end of their trajectories, such that these experience an obstruction to leave the plane [({\bf D}) in Fig.~\ref{fig:braiding3D}{\bf c}, and ({\bf B}) in Fig.~\ref{fig:braiding3D}{\bf d}].



\section{Conversion by braiding analysis in 3D}
We present here the numerical data and discuss the scenarios when two principal WPs collide within a $C_2\mathcal{T}$ symmetric plane depending on their braiding with adjacent WPs. We organize the braiding protocol such that the obstruction to leave the symmetric plane happens for the principal WPs. 

\subsubsection{WP location within the symmetric plane}

In Fig.~\ref{fig:protocol_3D_data} we draw the product of the magnitude of the two gaps, principal and adjacent, over the 2D Brillouin zone at the symmetric plane $k_3=0$. Lighter (darker orange) color indicates larger (smaller) gaps (principal and adjacent combined). The dark spots indicate the location of WPs. 

Fig.~\ref{fig:protocol_3D_data}{\bf a} ({\bf b}) corresponds to the process of Fig.~5{\bf c} (respectively, {\bf d}) of the main text. Following the main text, we label the processes between two WPs that meet as ({\bf A}), ({\bf B}), ({\bf C}), ({\bf D}), and ({\bf E}), see below and in Fig.~5 of the main text.   

In Fig.~\ref{fig:protocol_3D_data}{\bf a} we start (panel~1) with the creation of two secondary WPs of equal chirality within the symmetric plane ({\bf E}). Then we collide them after they run, each in opposite direction, through a non-contractible loop of the Brillouin zone (panels~2--3). Since there has been no braiding for them, they can leave the plane, one above and one below ({\bf A}). A pair of principal WPs of opposite chirality is now created ({\bf C}) (panel~4). We make them collide after they run, each in opposite direction, along a non-contractible loop that crosses the past trajectory of the adjacent WPs (panels~5--7). Due to the nontrivial frame-rotation charge they acquired through the braiding with the adjacent WPs, these do not annihilate and bounce back within the symmetric plane ({\bf D}) (panel~8). 


In Fig.~\ref{fig:protocol_3D_data}{\bf b} we start (panel~1) with the creation of two principal WPs of equal chirality within the symmetric plane ({\bf E}). Two adjacent WPs of opposite chirality are then created ({\bf C}) (panel~2). We collide the adjacent WPs after they run, each in opposite direction, through a non-contractible loop of the Brillouin zone (panels~3--4). Since there has been no braiding for them, they can leave the plane through annihilation ({\bf C}). We then collide the principal WPs after they run, each in opposite direction, through a non-contractible loop (panels~5--6). Since their trajectory crosses the past trajectory of the adjacent WPs they acquired a nontrivial frame-rotation charge which forbids them to leave the symmetric plane, so that they bounce away within the plane ({\bf B}) (panel~7). 

\subsubsection{Values of the tight-binding parameters}

The tight-binding parameters for the protocol of Fig.~\ref{fig:protocol_3D_data}{\bf a}, and  Fig.~\ref{fig:protocol_3D_data}{\bf b}, are given in Table \ref{TB_table_I}~A, and Table \ref{TB_table_I}~B, respectively. The tight-binding parameters of Table \ref{TB_table_I} are themselves defined in terms of control parameters which values determine the WP configuration at a given ``time'' of the protocol. We list the values of the control parameters corresponding to the snapshots of Fig.~\ref{fig:protocol_3D_data}{\bf a}, and  Fig.~\ref{fig:protocol_3D_data}{\bf b}, in Table \ref{TB_table_II}~A, and Table \ref{TB_table_II}~B, respectively. 



\subsubsection{Chirality of each pair of WPs}

The identification of the processes ({\bf A}, {\bf B}, {\bf C}, {\bf D}, {\bf E}) requires the computation of the chiral charge of the WP pair involved. We show in Fig.~\ref{fig:chirality_3D} the in-plane band structure with a pair of WPs (left column) and the computation of the corresponding chirality (right column) at snapshots of the 3D braiding protocol Fig.~\ref{fig:protocol_3D_data}. The chirality is obtained as the winding number of the flow of Berry phase as we sweep a base loop over a sphere wrapping the WP pair from a north pole (NP) above the symmetry plane to a south pole (SP) underneath the symmetric plane, and with the equator (E) defining a loop within the symmetric plane (visible as the black line on the left column). 

Fig.~\ref{fig:chirality_3D}{\bf a} captures the adjacent WP pair between ({\bf E}) and ({\bf A}) of Fig.~\ref{fig:protocol_3D_data}{\bf a}, giving a chirality of $+2$, i.e. the WPs have equal chirality. Fig.~\ref{fig:chirality_3D}{\bf b} captures the principal WP pair between ({\bf C}) and ({\bf D}) of Fig.~\ref{fig:protocol_3D_data}{\bf a}, revealing that these have opposite chirality (since the total chirality is zero). 

Fig.~\ref{fig:chirality_3D}{\bf c} captures the adjacent WP pair between ({\bf C}) and ({\bf C}) of Fig.~\ref{fig:protocol_3D_data}{\bf b}, revealing that they have an opposite chirality. Fig.~\ref{fig:chirality_3D}{\bf d} captures the principal WP pair between ({\bf E}) and ({\bf B}) of Fig.~\ref{fig:protocol_3D_data}{\bf b}, revealing that these have equal chirality.
 
\subsubsection{Stable critical points} 
 
Finally, we show in Fig.~\ref{fig:critical_points_3D}{\bf a}, and {\bf b}, the band structures at the stable critical points of Fig.~\ref{fig:protocol_3D_data}{\bf a}, and Fig.~\ref{fig:protocol_3D_data}{\bf b} respectively, i.e. when the two principal WPs meet exactly before to bounce away through the process ({\bf D}), and ({\bf B}) respectively. The band structure shows a two-dimensional slice of the 3D band structures with one direction taken within the symmetric plane and the other direction taken along the vertical axis $(001)$ for $k_3\in[0,1]$. 







%%%%%%%%%%%%%%%%%%%% FIGURE HERE %%%%%%%%%%%%%%%%%%%%
\begin{figure*}[htpb!]
\centering
\begin{tabular}{l}
{\bf a} \\
\begin{tabular}{llll} 
	1.\includegraphics[width=0.22\linewidth]{figs/3D_braiding_c_1.pdf} &
	2.\includegraphics[width=0.22\linewidth]{figs/3D_braiding_c_2.pdf} &
	3.\includegraphics[width=0.22\linewidth]{figs/3D_braiding_c_3.pdf} &
	4.\includegraphics[width=0.22\linewidth]{figs/3D_braiding_c_4.pdf} \\
	5.\includegraphics[width=0.22\linewidth]{figs/3D_braiding_c_5.pdf} &
	6.\includegraphics[width=0.22\linewidth]{figs/3D_braiding_c_6.pdf} &
	7.\includegraphics[width=0.22\linewidth]{figs/3D_braiding_c_7.pdf} &
	8.\includegraphics[width=0.22\linewidth]{figs/3D_braiding_c_8.pdf} 
\end{tabular}\\
{\bf b}\\
\begin{tabular}{llll} 
	1.\includegraphics[width=0.22\linewidth]{figs/3D_braiding_d_1.pdf} &
	2.\includegraphics[width=0.22\linewidth]{figs/3D_braiding_d_2.pdf} &
	3.\includegraphics[width=0.22\linewidth]{figs/3D_braiding_d_3.pdf} &
	4.\includegraphics[width=0.22\linewidth]{figs/3D_braiding_d_4.pdf} \\
	5.\includegraphics[width=0.22\linewidth]{figs/3D_braiding_d_5.pdf} &
	6.\includegraphics[width=0.22\linewidth]{figs/3D_braiding_d_6.pdf} &
	7.\includegraphics[width=0.22\linewidth]{figs/3D_braiding_d_7.pdf} &
\end{tabular}\\
\end{tabular}\\
\caption{\textsf{\textbf{3D braiding protocol.} Product of the magnitude of the two gaps, principal and adjacent, over the 2D Brillouin zone at the symmetric plane $k_3=0$. Lighter (darker orange) color indicates larger (smaller) gaps (principal and adjacent combined). The dark spots indicate the location of WPs. {\bf a} Numerical data corresponding to the process of Fig.~5{\bf c} of the main text with the successive steps ({\bf E}), and ({\bf A}) for the adjacent WPs, and then ({\bf C}), and ({\bf D}) for the principal WPs. {\bf b} Numerical data corresponding to the process of Fig.~5{\bf d} of the main text with the successive steps ({\bf E}) for principal WPs, ({\bf C}) for adjacent WPs, and again ({\bf C}) for adjacent WPs, and eventually ({\bf B}) for principal WPs.}}
\label{fig:protocol_3D_data} 
\end{figure*}
%%%%%%%%%%%%%%%%%%%% FIGURE HERE %%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%% FIGURE HERE %%%%%%%%%%%%%%%%%%%%
\begin{figure}[htpb!]
\centering
\begin{tabular}{ll}
{\bf a} & \\
	\includegraphics[width=0.55\linewidth]{figs/chirality_c_E_A_BS.pdf} & 
	\includegraphics[width=0.45\linewidth]{figs/chirality_c_E_A.pdf} \\
	{\bf b} & \\
	\includegraphics[width=0.55\linewidth]{figs/chirality_c_C_D_BS.pdf} & 
	\includegraphics[width=0.45\linewidth]{figs/chirality_c_C_D.pdf} \\
{\bf c} & \\
		\includegraphics[width=0.55\linewidth]{figs/chirality_d_C_C_BS.pdf} & 
	\includegraphics[width=0.45\linewidth]{figs/chirality_d_C_C.pdf} \\
	{\bf d} &  \\
	\includegraphics[width=0.55\linewidth]{figs/chirality_d_E_B_BS.pdf} & 
	\includegraphics[width=0.45\linewidth]{figs/chirality_d_E_B.pdf} 
\end{tabular} 
\caption{\textsf{\textbf{Weyl point pair chirality.} Left column: Band structure within the symmetric plane with the pairs of Weyl points (WPs) involved in the processes ({\bf A}), ({\bf B}), ({\bf C}), ({\bf D}), and ({\bf E}) of Fig.~\ref{fig:protocol_3D_data}. Right column: Flow of Berry phase over a base sphere, wrapping each pair of WPs, from the north pole (NP), above the symmetric plane, to the south pole (SP), underneath the plane, and with the equator (E) intersecting the plane (black circle in the figures on the left). {\bf a} WP pair between ({\bf E}) and ({\bf A}) of Fig.~\ref{fig:protocol_3D_data}{\bf a}. {\bf b} WP pair between ({\bf C}) and ({\bf D}) of Fig.~\ref{fig:protocol_3D_data}{\bf a}. {\bf c} WP pair between ({\bf C}) and ({\bf C}) of Fig.~\ref{fig:protocol_3D_data}{\bf b}. {\bf d} WP pair between ({\bf E}) and ({\bf B}) of Fig.~\ref{fig:protocol_3D_data}{\bf b}.}}
\label{fig:chirality_3D} 
\end{figure}
%%%%%%%%%%%%%%%%%%%% FIGURE HERE %%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%% FIGURE HERE %%%%%%%%%%%%%%%%%%%%
\begin{figure}[htpb!]
\centering
\begin{tabular}{l}
{\bf a}\\
	\includegraphics[width=0.6\linewidth]{figs/3D_braiding_c_BS.pdf} \\
	{\bf b}\\
	\includegraphics[width=0.6\linewidth]{figs/3D_braiding_d_BS.png} 
\end{tabular}
\caption{\textsf{\textbf{Stable critical points of the 3D braiding protocol.} {\bf a} Band structure at $k_1=0.13\pi$ for $(k_2,k_3)\in [-1,1]\times [0,1]$ at the critical point ({\bf D}) of the braiding protocol Fig.~\ref{fig:protocol_3D_data}{\bf a}. {\bf b} Band structure at $k_2=0.31\pi$ for $(k_1,k_3)\in [-1,1]\times [0,1]$ at the critical point ({\bf B}) of the braiding protocol Fig.~\ref{fig:protocol_3D_data}{\bf b}. }}
\label{fig:critical_points_3D} 
\end{figure}
%%%%%%%%%%%%%%%%%%%% FIGURE HERE %%%%%%%%%%%%%%%%%%%%

 
\begin{table*}[htpb!]
\centering
\caption{\textsf{\label{TB_table_I} Tight-binding parameters for the 3D braiding protocol of Fig.~\ref{fig:protocol_3D_data} parameterized as functions of the control parameters $\{p_0,p_1,p_2,p_3,p_4,p_5,p_6\}$, see Table \ref{TB_table_II}. \vspace{0.5cm}
}}
%\begin{tabular*}{\linewidth}{c @{\extracolsep{\fill}} c c }
\begin{tabular}{l}
A.~Tight-binding parameters for Fig.~\ref{fig:protocol_3D_data}{\bf a}. \\
\begin{tabular}{lll}
\hline \\
$a^0_0 = 0.5 p_0 $ & 
	$b^u_0 = 0$ &
		$ f^0_0 = 0.85 e^{-i 0.1 \pi}$ \\
$a^0_1 = i(0.45 p_3 + 0.045 p_4) $ & 
	$ d^0_0 = 3.33  $ &
		$ f^0_1 = i ( p_1  + 0.35 p_3) e^{i 0.2 \pi }$ \\
$a^0_2 = -0.3 p_3 $ & 
	$ d^0_1 = -0.1 p_3$ &
		$ f^0_2 = (-0.125 p_1  - 0.3 p_3 - 0.05 p_4) e^{i 0.2 \pi}$ \\
$a^0_3 = -0.2 p_3 $ & 
	$d^0_2 = 0.2  e^{i  0.1 \pi} p_3 $ &
		$ f^0_3 =( 0.5 p_1 - 0.03 p_4) e^{i 0.2 \pi }$ \\
$a^0_4 = 0.1 p_3 $ & 
	$d^0_3 = (0.2 p_3 + 0.029 p_4 ) e^{-i 0.099 \pi} $ &
		$ f^0_4 = -0.25 p_3 $ \\
$b^0_0 = 0$ & 
	$d^0_4 = -0.2  e^{-i 0.2 \pi} p_3$ &
		$ f^0_5 = 0.55  p_3 - 0.7 p_5 $  \\
$b^0_1 =0$ & 
	$d^0_5 = 0.333 e^{-i 0.45 \pi} p_2 $ & 
		$ f^0_6 =  0 $  \\
$b^0_2 =-0.03 p_4$ & 
	$d^0_6 = 0 $ &
		$ f^0_7 = 0 $ \\
$b^0_3 =0$ &   
	$d^0_7 = i 0.667   e^{- i 0.45 \pi} p_2 $ &
		 $ f^0_8 =  0.5 p_3 + 0.05 p_4 $ \\
$b^0_4 =-0.1 p_3$ & 
	$d^0_8 = -0.05  e^{-i 0.2 \pi } p_3 $ &  $a^u_0 = 0.25 p_0$
%\end{tabular*}
\end{tabular} \\
\\
B.~Tight-binding parameters for Fig.~\ref{fig:protocol_3D_data}{\bf b}. \\
\hline \\
\begin{tabular}{lll}
$a^0_0 = 4.5 - 3.5 p_3$ & 
	$b^u_0 = 0$ &
		$ f^0_0 = 1.25 $ \\
$a^0_1 = 0 $ & 
	$ d^0_0 = 2.67 e^{- i 0.35 \pi} $ &
		$ f^0_1 = i ( 0.5 p_1 - 0.1 p_4 ) e^{-i 0.15 \pi} $ \\
$a^0_2 = 0 $ & 
	$ d^0_1 = -1.333 p_4 $ &
		$ f^0_2 = 0.125 p_1  $ \\
$a^0_3 = - p_4 $ & 
	$d^0_2 = -0.1667 p_4 $ &
		$ f^0_3 = (0.5 p_1 - 0.45 p_4 ) e^{-i 0.15 \pi}$ \\
$a^0_4 = 0.35 p_4 $ & 
	$d^0_3 = ( -0.1667 p_2 - 0.2667 p_4 + 0.0005 p_5 e^{-i  0.0015 \pi} ) $ &
		$ f^0_4 = -0.55 p_3 $ \\
$b^0_0 = 0$ & 
	$d^0_4 = 0.1667 p_4 $ &
		$ f^0_5 = -0.5 p_3 - 0.001667 p_5 $  \\
$b^0_1 = -0.5 p_3$ & 
	$d^0_5 = ( 0.333 p_2  - 0.000333 p_5 ) e^{i 0.2 \pi}$ & 
		$ f^0_6 =  -0.3 p_3 $  \\
$b^0_2 =0$ & 
	$d^0_6 = 0.1 p_5 e^{-i 0.06 \pi} $ &
		$ f^0_7 = 0.55 p_4 $ \\
$b^0_3 = 0.5 p_4 $ &   
	$d^0_7 = i ( 0.667 p_2 + 0.0667 p_5) e^{i 0.2 \pi} $ &
		 $ f^0_8 =  0.3 p_3 $ \\
$b^0_4 = 0.5 p_4 $ & 
	$d^0_8 = 0.333 p_6 $ & $a^u_0 = 2.25 - 1.75 p_3$
%\end{tabular*}
\end{tabular}
\end{tabular}
\end{table*} 


\begin{table*}[htpb!]
\centering
\caption{\textsf{\label{TB_table_II} Values of the control parameters $\{p_0,p_1,p_2,p_3,p_4,p_5,p_6\}$ entering Table \ref{TB_table_I} and corresponding to the snapshots of Fig.~\ref{fig:protocol_3D_data}. \vspace{0.5cm}
}}
%\begin{tabular*}{\linewidth}{c @{\extracolsep{\fill}} c c }
%\end{tabular*}
\begin{tabular}{l}
A.~Control parameters for the snapshots of Fig.~\ref{fig:protocol_3D_data}{\bf a}.  \\
\begin{tabular}{l | llllll}
\hline 
1.& $p_0 = 10.4 $ & 
	$p_1 = 0.6 $ &
		$p_2 = 1 $ &
			$p_3 = 0 $ & 
				$ p_4 = 0 $ &
					$ p_5 = 0 $ \\
2.& $p_0 = 10.4 $ & 
	$p_1 = 1 $ &
		$p_2 = 1 $ &
			$p_3 = 0 $ & 
				$ p_4 = 0 $ &
					$ p_5 = 0 $ \\
3.& $p_0 = 10.4 $ & 
	$p_1 =  1.4 $ &
		$p_2 = 1 $ &
			$p_3 = 0 $ & 
				$ p_4 = 0 $ &
					$ p_5 = 0 $ \\
4.& $p_0 = 6.76 $ & 
	$p_1 =  2 $ &
		$p_2 = 1 $ &
			$p_3 = 0 $ & 
				$ p_4 = 0 $ &
					$ p_5 = 0 $ \\
5.& $p_0 = 5.2 $ & 
	$p_1 =  2 $ &
		$p_2 = 1 $ &
			$p_3 = 0 $ & 
				$ p_4 = 0 $ &
					$ p_5 = 0 $ \\
6.& $p_0 = 5.2 $ & 
	$p_1 =  2 $ &
		$p_2 = 1 $ &
			$p_3 = 1 $ & 
				$ p_4 = 0 $ &
					$ p_5 = 0 $ \\
7.& $p_0 = 5.2 $ & 
	$p_1 =  2 $ &
		$p_2 = 1 $ &
			$p_3 = 1 $ & 
				$ p_4 = 1 $ &
					$ p_5 = 0 $ \\
8.& $p_0 = 5.2 $ & 
	$p_1 =  2 $ &
		$p_2 = 1 $ &
			$p_3 = 1 $ & 
				$ p_4 = 1 $ &
					$ p_5 = 1 $ 
\end{tabular} \\
\\
B.~Control parameters for the snapshots of Fig.~\ref{fig:protocol_3D_data}{\bf b}. \\
\hline 
\begin{tabular}{l | llllll}
1.& $p_1 = 1.6  $ & 
	$p_2 =  1 $ &
		$p_3 = 0 $ &
			$p_4 = 0 $ & 
				$ p_5 = 0 $ &
					$ p_6 = 0 $ \\
2.& $p_1 = 2.48 $ & 
	$p_2 =  1.24 $ &
		$p_3 = 0.3 $ &
			$p_4 = 0 $ & 
				$ p_5 = 0 $ &
					$ p_6 = 0 $ \\
3.& $p_1 = 2.8 $ & 
	$p_2 =  1.4 $ &
		$p_3 = 0.5 $ &
			$p_4 = 0 $ & 
				$ p_5 = 0 $ &
					$ p_6 = 0 $ \\
4.& $p_1 = 3.12 $ & 
	$p_2 =  1.56 $ &
		$p_3 = 0.7 $ &
			$p_4 = 0 $ & 
				$ p_5 = 0 $ &
					$ p_6 = 0 $ \\
5.& $p_1 = 3.6 $ & 
	$p_2 =  1.8 $ &
		$p_3 = 1 $ &
			$p_4 = 0.5 $ & 
				$ p_5 = 0 $ &
					$ p_6 = 0 $ \\
6.& $p_1 = 3.6 $ & 
	$p_2 =  1.8 $ &
		$p_3 = 1 $ &
			$p_4 = 1 $ & 
				$ p_5 = 1 $ &
					$ p_6 = 0 $ \\
7.& $p_1 = 3.6 $ & 
	$p_2 =  1.8 $ &
		$p_3 = 1 $ &
			$p_4 = 1 $ & 
				$ p_5 = 1 $ &
					$ p_6 = 1 $ 
%\end{tabular*}
\end{tabular}
\end{tabular}
\end{table*}            
  
  
  
\appendix


\section{Extra relations}

Let us write $\hat{h}_{ij}$ the symmetric matrix with the single non-zero elements, $[\hat{h}_{ij}]_{kl}  = \delta_{ik}\delta_{jl} + \delta_{il}\delta_{jk} = [\hat{h}_{ji}]_{kl} $ if $i\neq j$, and $[\hat{h}_{ii}]_{kl}  = \delta_{ik} \delta_{il}$. The conversion from the $\hat{h}$'s matrices to the gamma matrices then reads
\begin{equation}
    \begin{aligned}
        \gamma_{00} &= \dfrac{1}{4} \left( \hat{h}_{11} + \hat{h}_{22} +  \hat{h}_{33} +\hat{h}_{44} \right),\\
        \gamma_{01} &= \dfrac{1}{4} \left( \hat{h}_{12} + \hat{h}_{34} \right),\\
        \gamma_{03} &= \dfrac{1}{4} \left( \hat{h}_{11} - \hat{h}_{22} +  \hat{h}_{33} - \hat{h}_{44} \right),\\
        \gamma_{10} &= \dfrac{1}{4} \left( \hat{h}_{13} + \hat{h}_{24}  \right),\\
        \gamma_{30} &= \dfrac{1}{4} \left( \hat{h}_{11} + \hat{h}_{22} -  \hat{h}_{33} - \hat{h}_{44} \right),\\
        \gamma_{11} &= \dfrac{1}{4} \left( \hat{h}_{14} + \hat{h}_{23} \right),\\
        \gamma_{13} &= \dfrac{1}{4} \left( \hat{h}_{13} - \hat{h}_{24}  \right),\\
        \gamma_{22} &= \dfrac{1}{4} \left(  -\hat{h}_{14} + \hat{h}_{23}   \right),\\
        \gamma_{31} &= \dfrac{1}{4} \left(\hat{h}_{12} - \hat{h}_{34} \right),\\
        \gamma_{33} &= \dfrac{1}{4} \left( \hat{h}_{11} - \hat{h}_{22} -\hat{h}_{33} +\hat{h}_{44}  \right).
    \end{aligned}
\end{equation}


\subsection{UNUSED FIGURE!!!}
%%%%%%%%%%%%%%%%%%%% FIGURE HERE %%%%%%%%%%%%%%%%%%%%
\begin{figure*}[htpb!]
\centering
\begin{tabular}{llll} 
1. & 2. & 3. & 4.\\
	\includegraphics[width=0.22\linewidth]{4B_11/t_0110.pdf} &
	\includegraphics[width=0.22\linewidth]{4B_11/t_0151.pdf} &
	\includegraphics[width=0.22\linewidth]{4B_11/t_0160.pdf} &
	\includegraphics[width=0.22\linewidth]{4B_11/t_0198.pdf} \\
5. & 6. & 7. & 8.\\
	\includegraphics[width=0.22\linewidth]{4B_11/t_0211.pdf} &
	\includegraphics[width=0.22\linewidth]{4B_11/t_0500.pdf} &
	\includegraphics[width=0.22\linewidth]{4B_11/t_0610.pdf} &
	\includegraphics[width=0.22\linewidth]{4B_11/t_0701.pdf} 
\end{tabular}
\caption{\textsf{\textbf{4-band $\vec{\chi} = (1,1)$.} Debraiding  }}
\label{fig:4B_11_debraiding} 
\end{figure*}
%%%%%%%%%%%%%%%%%%%% FIGURE HERE %%%%%%%%%%%%%%%%%%%%


